Solon: Communication-efficient Byzantine-resilient Distributed Training via Redundant Gradients

There has been a growing need to provide Byzantine-resilience in distributed model training. Existing robust distributed learning algorithms focus on developing sophisticated robust aggregators at the parameter servers, but pay less attention to balancing the communication cost and robustness. In this paper, we propose Solon, an algorithmic framework that exploits gradient redundancy to provide communication efficiency and Byzantine robustness simultaneously. Our theoretical analysis shows a fundamental trade-off among computational load, communication cost, and Byzantine robustness. We also develop a concrete algorithm to achieve the optimal trade-off, borrowing ideas from coding theory and sparse recovery. Empirical experiments on various datasets demonstrate that Solon provides significant speedups over existing methods to achieve the same accuracy, over 10 times faster than Bulyan and 80% faster than Draco. We also show that carefully designed Byzantine attacks break Signum and Bulyan, but do not affect the successful convergence of Solon.

==> Figure/Conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}\label{Sec:SOLON:Conclusion}
\vspace{-0.1in}

In this paper, we propose \systemnameSolon{}, %\footnote{Our code and data will be available at \url{https://github.com/chenleshang/solon}}
a distributed training framework that simultaneously resists Byzantine attack and reduces communication overhead via algorithmic redundancy. 
We show that there is a fundamental trade-off between Byzantine-resilience, communication cost, and computational cost.
% In addition, \solon{ } utilizes a Vandermonde matrix-based  technique which achieves this trade-off.
Extensive experiments show that \solon{} provides significant speedups over existing methods, and consistently leads to successful convergence under different attacks. 

==> Figure/Experiment.tex <==
\vspace{-0.1in}
\section{Experiments}\label{Sec:SOLON:Experiment}
\vspace{-0.1in}
Now we present an empirical study on \solon{} compared with several existing methods including \draco{}~\cite{DRACO}, \bulyan{}~\cite{guerraoui2018hidden}, and \signum{}~\cite{bernstein2018signsgd}. 
Across diverse ML models trained on real world datasets, we have found 1) that \solon{} results in significant speedups over existing methods, including $10\times$ faster than \bulyan{} and $80\%$ faster than \draco{} while reaching the same accuracy, and  2) that \solon{} consistently leads to successful convergence for all Byzantine attacks considered, while previous approaches may fail on different attacks (\eg \signum{} on constant attack, and \bulyan{} on "A little is enough" (ALIE) attack~\cite{ALIE2019}). 

\begin{table}[b]
\centering
\begin{minipage}{.58\linewidth}
    \medskip
    % \raggedleft
	\centering
	\caption{Summary of the datasets, models, and hyper-parameters used in our experiments.}
	\scalebox{0.95}{
	\begin{tabular}{cccc}
		\toprule Dataset
		& CIFAR-10 & SVHN & \makecell{WikiText-2}\bigstrut\\
		\midrule
		\midrule
		\# data points & 60,000 & 600,000 & 2,551,843 \bigstrut\\
		Model & ResNet-18 & VGG13-BN  & LSTM \bigstrut\\
% 		\# Classes & 10 & 10 & 10 \bigstrut\\
		\# Parameters & 11,173k & 9,923k  & 7,332k \bigstrut\\
		Optimizer & SGD & SGD &SGD \bigstrut\\
		%Learning Rate & 0.1 & 0.1 \bigstrut\\
		%Momentum & 0.9 & 0.9 \bigstrut\\
		%\signum{} LR & 5E-5 & 5E-5\bigstrut \\
		Batch Size & 120 & 120 & 60 \bigstrut\\
		\bottomrule
    	\end{tabular}
    	}%
    % 	\vspace{-2mm}
		\label{Tab:solon:DataStat}%
\end{minipage}
\hskip 10pt
% \hfill
\begin{minipage}{.37\linewidth}
% \raggedright
    \medskip
	\centering
% 	\vspace{0.3 cm}
    \caption{The size of gradients to transmit per worker before and after compression (MB, $10^6$ bytes). }
    \scalebox{0.86}{
	
	\begin{tabular}{cccc}
		\toprule Model & 
		  ResNet18 & VGG13 & LSTM \bigstrut\\
		\midrule
		\midrule
		Size & 89.6 & 79.4 & 58.8   \bigstrut\\
% 		$r_c=4$ & 22.4 & 19.84 & 34.4 \bigstrut\\
		$r_c=6$ & 14.9 & 13.2 & 9.78 \bigstrut\\
		$r_c=8$ & 11.2 & 9.92 & 7.35  \bigstrut\\
		$r_c=10$ & 8.96  & 7.94  & 5.88  \bigstrut\\
		
		\bottomrule
	\end{tabular}
	}%
% 	\vspace{-3mm}
	\label{Tab:compressionsize}
	\end{minipage}
	\vspace{-3mm}
\end{table}

\begin{figure}[t] 
\centering
\includegraphics[width=0.94\textwidth]{Figure/accu_iter_hour_legend_node50.pdf}\\
\vspace{-2mm}
\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_iter_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps,  constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_ALIE_node50_ResNet.pdf}}\\
\vspace{-3mm}
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_ALIE_node50_ResNet.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} and other baselines on ResNet-18 and CIFAR-10. (a)-(c): Comparison of test accuracy vs. the number of iterations between 
\solon{} $r_c=10$ and other methods under different attacks. (d)-(f): Test accuracy vs. running time of \solon{} and other methods. Vanilla SGD simply averages gradients received on PS and is tested without adversary. Accuracy may fluctuate occasionally due to randomness and lr adjustments.} }

\vspace{-5mm}
\label{fig:against-defense}
\end{figure}


\paragraph{Experimental setup.} 
We implement \solon{} in PyTorch~\cite{paszke2019pytorch} with MPI~\cite{DALCIN20051108}.
The experiments were conducted on a cluster of 50 real machines from Cloudlab  \cite{CloudlabDuplyakin} with 1 Gbps network speed and 100 virtual compute nodes. We trained three large scale models, namely, ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10}, VGG13-BN~\cite{VGGverydeepconv} on SVHN~\cite{svhn}, and a two-layer stacked LSTM \cite{LSTMnips96} (nhid=200) on WikiText-2~\cite{wikitext-2}, respectively.  %and WRN-22-8~\cite{WRNwiderangenet} on on Fashion-MNIST~\cite{fashionmnist}, respectively. 
The details are summarized in Table \ref{Tab:solon:DataStat}.
For comparison with \solon{}, we also evaluate two robust aggregator-based approches, \bulyan{}, \signum{}, and an algorithmic redundancy-based approach, \draco{}.  \solon{} splits the virtual machines evenly into 5 groups, each with 20 redundant machines. To compare with the best possible performance of \draco{}, we set the $r=11$ and only use 5 groups for \draco{} to reduce its communication overhead. 
More details are in the appendix.


\vspace{-2mm}
\paragraph{Attacks.} We use three different attacks:  reverse gradient,  constant, and ALIE (``A little is enough''~\cite{ALIE2019}). 
In the reverse gradient attack (rev-grad), Byzantine nodes always send $\kappa$ times the true gradient to the PS. 
In the constant attack, Byzantine nodes always send a constant multiple $c$ of the all-ones vector.
In the experiments shown, $\kappa = -100$ and $c=-100$.
%Since \signum{} is generally resilient to  flip sign attacks like rev-grad. 
%We set $\kappa = -100$ for the rev-grad attack and $c=-100$ for constant attack. 
In ALIE, Byzantine nodes use local information to estimate the mean and variance of the gradients computed at the other nodes, and then manipulate the gradient as $ \hat{\mu} + z \cdot \hat{\sigma}$ where $\hat{\mu}$ and $\hat{\sigma}$ are the mean and standard deviation of the gradients estimated by Byzantine nodes and $z$ is an adjustable hyper-parameter that adds an unnoticeable perturbation to disrupt the aggregation. In experiments, we set $z=1$.   
At each iteration, we randomly select $s = 5$ compute nodes as adversaries. 


\vspace{-2mm}
\paragraph{End to end performance.} We start by evaluating \solon{}'s end to end performance along with the baseline methods under different attacks, which is shown in Figure~\ref{fig:against-defense}.
We first note that previous approaches may result in significant accuracy loss under certain attacks. For example, \signum{}'s accuracy is 30\% worse than   the Byzantine-free vanilla SGD under constant attack (Figure~\ref{fig:against-defense}(b)), and ALIE attack leads a 50\% accuracy drops for \bulyan{} (Figure~\ref{fig:against-defense}(c)).
Nevertheless, across different attacks, \solon{} consistently converges and matches the accuracy performance of the vanilla SGD in a Byzantine-free environment. 
This is primarily due to \solon{}'s black box performance guarantee.



\begin{figure}[t]
\vspace{-4mm}
\centering

\subfigure[ResNet18, CIFAR-10]{\includegraphics[width=0.33\textwidth]{Figure/time_breakdown_4methods_RN18_node50.pdf}}
\subfigure[VGG13-BN, SVHN ]{\includegraphics[width=0.31\textwidth]{Figure/time_breakdown_4methods_node50_SVHN_revgrad.pdf}}
\subfigure[LSTM, WikiText-2]{\includegraphics[width=0.30\textwidth]{Figure/time_breakdown_4methods_RN18_node50_LSTM.pdf}}

\vspace{-3mm}
\caption{\footnotesize{Time breakdown per iteration of \solon{} $r_c=10$ and all baseline methods over three models+datasets under rev-grad. The types of attack will not affect most of the times. Notice that even if \signum{} is the fastest in time per iteration among those methods, and even faster than vanilla SGD, its accuracy is sacrificed and thus \solon{} still has the best convergence performance.}} 
\label{fig:timebreakdown}
\vspace{-5mm}
\end{figure}

\begin{figure}[t]
  \centering
  \subfigure[Speed up ($\times$) of \solon{}]{\includegraphics[width=0.42\textwidth]{Figure/solon_speedup_heatmap_node50_RN18.pdf}}
  \hskip 20pt
  \subfigure[Time breakdown of \solon{}]{\includegraphics[width=0.40\textwidth]{Figure/time_breakdown_solonrc_node50_RN18_fixn.pdf}}
  \vspace{-3mm}
  \caption{\footnotesize{(a) The speed up ($\times$) of \solon{}, $r_c=10$ vs other baselines on converging to certain test accuracy level on ResNet-18+CIFAR-10 under selected attacks. Values are approximation. $\infty$ means the method does not converge to the accuracy in the experiment. (b) Time breakdown of \solon{} by varying $r_c$, fixing $s$ with similar \# of compute nodes on ResNet-18 trained over the CIFAR-10 dataset (regardless of attacks). } }
  \vspace{-3mm}
  \label{fig:solonspeedup}
\end{figure}

\begin{figure}[ht] 
\centering

\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_iter_3000_revgrad_node50_LSTM.pdf}}
\hskip 20pt
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_hour_3000_revgrad_node50_LSTM.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} $r_c=10$ and other baselines on LSTM model trained over WikiText-2 dataset under reverse gradient attack, $s=5$. (a) Validation perplexity vs. \# iterations. (b) Validation perplexity vs. running time. }}
\label{fig:against-defense:appendix:LSTM}
\vspace{-3mm}
\end{figure}

Furthermore, \solon{} provides significant runtime speedups over existing methods.
For example, as shown in Figure \ref{fig:against-defense}(d), \solon{} converges faster than all the other Byzantine-resilient approaches. 
Its runtime performance even outperforms the vanilla SGD in a Byzantine-free environment.
This is primarily due to the communication efficiency of \solon{}. We observe a similar trend for the other two models (\eg LSTM under rev-grad attack shown in Figure \ref{fig:against-defense:appendix:LSTM}). 
Figure \ref{fig:solonspeedup}(a) gives a quantitative result of the speedups achieved by \solon{}.
To achieve a 90\% test accuracy, \solon{} obtains a speedup of 1.8$\times$ over \draco{} and 11$\times$ over \bulyan{} under the reverse gradient attack, while  \signum{} cannot reach 90\% accuracy. Other details and results can be found in the Appendix. 

\vspace{-2mm}
\paragraph{Per iteration cost.} 
Next, we dive into the per iteration cost of each approach.
As shown in Figure \ref{fig:timebreakdown}.
We note that \bulyan{} requires a significantly higher decoding time than all the other methods. 
This is probably because \bulyan{} deploys a computational expensive robust aggregator. 
Note that \solon{} reduces the communication cost by slightly increasing the computation and decoding complexity compared to \draco{}. Nevertheless, across all datasets and models considered in our experiments, \solon{} attains the fastest per iteration runtime.
This is because \solon{} largely reduces the communication cost, which is the bottleneck in a large cluster, and the extra computation and decoding cost is relatively small. 
\vspace{-2mm}
\paragraph{Effects of compression ratio.}
Finally we evaluate the effects of the compression ratio $r_c$ on \solon{}'s performance, as shown in Figure \ref{fig:solonspeedup}(b).
Here we vary compression rate $r_c$, fix attacks $s$, and change redundancy ratio $r$ accordingly. We keep the entire number of machines roughly at the same level by varying group numbers. 
Overall, as the compression ratio decreases, the communication cost increases almost linearly, and thus the total runtime.
This shows that \solon{} can be applied for different communication requirements with small extra overhead. 
In addition, we observe that the computation cost increases slightly when $r_c$ goes up, since the increase of $r_c$ will require an increase in the group batch size. The decode time also changes slightly. However, these are not major factors compared to communication. 

Other details can be found in the appendix.

In addition, we also evaluate the size of the gradients before and after compression, summarized in Table \ref{Tab:compressionsize}. 
Overall, \solon{} largely reduces the gradient size up to 10$\times$, depending on the specified compression ratio $r_c$.
In fact, \solon{} allows users to specify the compression ratio explicitly to satisfy different clusters' requirements. 


==> Figure/Introduction.tex <==
\section{Introduction}\label{Sec:SOLON:Intro}
%TODO
The growing size of datasets and machine learning models has led to many developments in distributed training using stochastic optimization~\cite{devlin2018bert,deng2009imagenet,sergeev2018horovod,dean2012large,dobriban2020wonder}.
One of the most widely used %distributed training
settings is the {\em parameter server (PS) model}~\cite{li2013parameter,li2014scaling,jiang2020unified}, 

where the gradient computation is partitioned among all compute nodes, typically using stochastic gradient descent (SGD) or its variants. A central parameter server then aggregates the calculated gradients from all compute nodes to update the global model. 


However, scaling PS models to large clusters introduces two challenges: guarding against \textit{Byzantine attacks} and managing  \textit{communication overhead}.
Byzantine attacks include erroneous gradients sent from unreliable compute nodes due to power outages, hardware or software errors, as well as malicious attacks. 
The communication overhead of sending gradients to the PS in large clusters can also be extremely high, potentially dominating the training time, ~\cite{dean2012large,alistarh2017qsgd,wen2017terngrad,Wang18Atomo, DRACO}, since the number of gradients sent is linear in the number of compute nodes. 
Although recent work has studied the problem of
%extensively studied how to protect against 
Byzantine attacks under the PS model~\cite{ALIE2019,guerraoui2018hidden,xie2020fall}, the communication overhead remains prohibitive. For example, ~\cite{blanchard2017machine,chen2017distributed,yin2018byzantine,AggregathorDamaskinosEGGR19} use {\em robust aggregators} at the PS to mitigate  unreliable gradients, 
while ~\cite{DRACO} introduces {\em algorithmic redundancy} to detect and remove Byzantine nodes. 
Robust aggregators are computationally
expensive due to their super-linear  (often quadratic) dependence on the number
of nodes. They also often have limited convergence guarantees under
Byzantine attacks, e.g., only establishing convergence in the limit, or only guaranteeing that the output of the aggregator has a positive inner product with the true gradient. 
They often require strong bounds on the dimension of the model.
Although algorithmic redundancy or coding-theoretic~\cite{Gradient_Coding, DRACO}
approaches offer strong convergence guarantees, these approaches have high communication overhead.

Thus, it remains an open question to simultaneously provide \textbf{\emph{Byzantine-resilience with strong guarantees and communication efficiency}} for distributed learning.





\begin{figure*}[t] 
\centering
\subfigure[Example of a \solon{} instance]{\includegraphics[width=0.6\textwidth]{Figure/intro_fig_2.pdf}}
% \hfill
\hskip 5pt
\subfigure[Performance of \solon{}]{\includegraphics[width=0.37\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet_w_errorbar.pdf}}
\vspace{-2mm}
\caption{\footnotesize{Demonstration of \solon{}. (a) gives an example of \solon{}, where the cluster consists of  four compute nodes.  (b) shows the runtime performance of \solon{} $r_c=10$ when training ResNet-18 on CIFAR-10 under rev-grad attack. Compared to various baselines, \solon{} converges faster and provides higher final accuracy.}}
\label{fig:RunningExample}
% \vspace{-2mm}
\end{figure*}

To address this problem, we propose \solon{}, a distributed training framework leveraging algorithmic redundancy to protect against Byzantine attacks, and ideas from sparse recovery~\cite{Prony} and coding theory~\cite{Gradient_Coding} to reduce communication overhead. 

The approach is as follows: 
In a Byzantine-free PS model with $P$ compute nodes and $B$ gradients to be computed, at each iteration
each of the $P$ nodes computes $B/P$ gradients, and sends them to the PS.  In \solon{}, gradients are computed redundantly to tolerate Byzantine failures; each node computes $rB/P$ gradients, incurring a {\em computational redundancy ratio} of $r$.  To reduce communication overhead, compressed gradients are sent to the PS.  For $d$-dimensional gradients, each node only sends a $d/r_c$-dimensional vector to the PS, where  $r_c$ is the {\em compression ratio}. 

We show that under worst-case adversarial conditions where the adversarial nodes have access to the complete data and gradients, and can send arbitrary results to the PS, there is a fundamental trade-off among Byzantine-resilience, communication overhead and computation cost. To tolerate $s$ Byzantine nodes, the redundancy ratio must satisfy $r\geq 2s+r_c$.
We provide a concrete encoding and decoding technique for \solon{} based on Vandermonde matrices and building on Prony's method from signal processing ~\cite{Prony,communciation_gradcoding_min_ye} that matches the optimal condition  $r= 2s+r_c$. 


\paragraph{Example.}
Figure \ref{fig:RunningExample}(a) shows
four two-dimensional gradient vectors, $g_1, g_2,g_3, g_4$, where gradients $g_i=(g_{i1},g_{i2})$ are in different colors.
To tolerate Byzantine workers, 
%\solon{} requires each compute node to compute redundant gradients. In Figure \ref{fig:RunningExample}(a), 
each node computes four gradients. 
However, instead of sending a two-dimensional vector to the PS, each node only sends a one-dimensional linear combination of the elements in the local gradients. For instance, worker 1 computes and sends the scalar $g_{11}+g_{12}+g_{21}+g_{32}+g_{41}+g_{42}$. Here, the redundancy ratio $r=4$ and the compression ratio $r_c=2$. The PS uses a decoding scheme presented in Section \ref{sec:solon}. Therefore \solon{} can recover the correct gradient with one Byzantine worker ($4 \geq 2\times 1 + 2$). 
\qed


We implemented \solon{} in Pytorch and conducted extensive experiments on a large cluster.  Our results show that
\solon{} can provide significant speedups across various ML models and datasets over existing methods, such as \bulyan{} \cite{guerraoui2018hidden} and \draco{}~\cite{DRACO}, shown in Figure \ref{fig:RunningExample}(b) using ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10} under a reverse gradient attack. 
In addition, 
\solon{} successfully defends against strong Byzantine attacks such as ``A little is enough'' (ALIE)~\cite{ALIE2019}, on which some methods such as \bulyan{} and \signum{} \cite{bernstein2018signsgd} fail to converge or result in significant accuracy loss, see Section \ref{Sec:SOLON:Experiment}. 


\vspace{-0.1in}
\paragraph{Contributions.}   Our contributions include:
\vspace{-0.1in}
\begin{enumerate}
    \item \solon{}, a distributed training framework that exploits algorithmic redundancy to simultaneously provide Byzantine-resilience and communication efficiency. 
    \vspace{-0.07in}
    \item Optimal trade-offs between Byzantine resilience, communication overhead, and computational cost. 
    \vspace{-0.07in}
    \item A concrete encoding and decoding mechanism, which is provably efficient and  achieves this optimal trade-off.
    \vspace{-0.07in}
    \item Extensive experiments which show that \solon{} exhibits significant speedups as well as strong Byzantine-resilience over previous approaches.   
\end{enumerate}

The \solon{} framework can be used for any distributed algorithm which requires the sum of multiple functions, including gradient descent, SVRG \cite{johnson2013accelerating}, coordinate descent, and projected or accelerated versions of these algorithms. However, in this paper, we focus on mini-batch SGD.
The rest of the paper is organized as follows: Section \ref{Sec:SOLON:relatedwork} discusses related work. %, and Section 
Section \ref{sec:solon} presents the \solon{} framework and theoretical guarantees. Experimental results are given in Section \ref{Sec:SOLON:Experiment}. 


\section{Related work}
\label{Sec:SOLON:relatedwork}
Byzantine fault tolerance against worst-case and/or adversarial failures such as system crashes, power outages, software bugs, and adversarial agents that exploit security flaws has been extensively studied since the 1980s~\cite{lamport2019byzantine}. In distributed machine learning, these failures may appear when a subset of compute nodes returns to the PS erroneous updates. It is well understood that first-order methods, such
as gradient descent or mini-batch SGD, are not robust to Byzantine errors; even a single erroneous update can introduce arbitrary errors to the optimization variables~\cite{blanchard2017machine,chen2017distributed}. At the same time, distributed model training suffers from communication overhead due to frequent gradient updates transmitted between compute nodes~\cite{LargeScaleDeepNet_Dean12,mcmahan2017communication,li2014communication,konevcny2016federated,dobriban2020wonder,dobriban2021distributed}. \solon{} aims at improving both Byzantine-resilience and communication-efficiency in distributed model training.

More recently, attention has turned to Byzantine-resilient distributed machine learning techniques.  Results show that while average-based gradient methods are susceptible to adversarial nodes, robust gradient aggregation methods can, in some cases, achieve better convergence while being robust to some attacks~\cite{chen2017distributed,el2019sgd,blanchard2017machine,xie2018zeno,xie2020fall,blanchard2017machine,yin2018byzantine,guerraoui2018hidden,jaggilearningfromhistory}. Despite
theoretical guarantees, the proposed algorithms often only ensure
a weak form of resilience against Byzantine failures, and can fail against strong Byzantine attacks~\cite{guerraoui2018hidden,xie2020fall,ALIE2019}. Another line of work proposes to use algorithmic redundancy to attain black-box Byzantine-resilience guarantees. However, many of these techniques require redundant computation from compute nodes (such as \draco{}~\cite{DRACO}) or place a heavy computation overhead on the PS (such as
\bulyan{}~\cite{guerraoui2018hidden}). Furthermore, they introduce a heavy communication overhead. \cite{detox2019} interpolates between \draco{} and robust aggregation methods for faster computation on both compute nodes and the PS. However, it does not mitigate the communication bottleneck, whereas \solon{} introduces both black-box Byzantine-resilience guarantee and communication-efficiency. 

Communication-efficient distributed machine learning has gained a lot of attention. Various methods propose to use gradient compression, \eg via quantization~\cite{seide20141,alistarh2016qsgd,wen2017terngrad,suresh2017distributed} or sparsification~\cite{stich2018sparsified,Wang18Atomo,lin2017deep,vogels2019powersgd,agarwal2020accordion} to enhance the communication efficiency. These methods massively compress the gradients, however, their Byzantine-resilience is not clear.

The methods that are the most similar to \solon{} are \signum{}~\cite{bernstein2018signsgd} and the one proposed in~\cite{ghosh2020communication}. These methods introduce both communication-efficiency and Byzantine-resilience, however their Byzantine-resilience guarantees are not as strong as for \solon{} in theory, i.e. they typically use lossy compression for coding and decoding schemes, which only achieve approximated recovery under certain attacks.  

==> Figure/Theory.tex <==

\section{\solon{}}
\label{sec:solon}
	\vspace{-0.1in}

In this section we give an overview of the \solon{} framework, discuss constraints on the encoding and decoding functions, and define optimal coding schemes.

The proofs are left to the appendix.

\subsection{Preliminaries}	\vspace{-0.1in}

\paragraph{Basic notations.}
For a matrix $\mathbf{A}$, let $\mathbf{A}_{i,j}$, $\mathbf{A}_{i,\cdot}$, and $\mathbf{A}_{\cdot, j}$ denote entries, rows, and columns, respectively. More generally, $\mathbf{A}_{S,T}$ is the submatrix of $\mathbf{A}$ with rows indexed by  $S$ and columns indexed by $T$. The Hadamard, or elementwise, product $\mathbf{A} \odot \mathbf{B}$ of two matrices of the same size has entries $(\mathbf{A}\odot \mathbf{B})_{i,j} = \mathbf{A}_{i,j}\mathbf{B}_{i,j}$. Let $m$ be the dimension of the data, $n$ be the size of the training set, and $\mathbf{x}_i\in\mathbb{R}^m$, $i=1,\ldots,m$ be the data points. Let $\ell(\cdot;\cdot)$ be the loss function, $d$ be the model dimension, and ${\bf w}\in\mathbb{R}^d$ be the model parameters.  Let $\mathbf{1}_m$ and $\mathbf{1}_{n\times m}$ be the $m\times 1$ vector, and $n\times m$ matrix, of all ones, respectively. Similarly, let $\mathbf{0}_{m}, \mathbf{0}_{n\times m}$ contain zeros.  The empirical risk minimization (ERM) \cite{NIPS1991ERM,vapnik2013nature} objective is: 
$\min_{{\bf w}} {n}^{-1}\sum_{i=1}^n \ell({\bf w};\mathbf{x}_i).$
The most common current approach is to use first-order stochastic optimization to solve this, in particular mini-batch stochastic gradient descent (SGD). Starting at an initial point ${\bf w}_0$, we iterate 
${\bf w}_k = {\bf w}_{k-1} - \gamma/|S_k| \sum_{i \in S_k}\nabla\ell_{\bf w}({\bf w}_{k-1}; \mathbf{x}_{i}),$
where $S_k \subseteq \{1,\ldots, n\}$ is a random subset of size $B$ and $\gamma>0$ is the learning rate.

We relabel $S_k$ to $\{1,\ldots, B\}$ and denote $\nabla \ell({\bf w}_{k-1};\mathbf{x}_i)$ by $\mathbf{g}_i$. 

\paragraph{Distributed learning.}
We aim to compute $\mathbf{g}=\sum_{i = 1}^B \mathbf{g}_i$ in a distributed, {\it adversary-resistant}, and {\it communication efficient} manner. We consider a distributed training model where gradient computations are partitioned across $P$ compute nodes at each iteration. These operate on a potentially reduced dimension $d_c$ for communication efficiency, and we let the gradient \emph{compression ratio} be $\smash{r_c \triangleq d/d_c}$. After computing and summing up their assigned gradients, each node sends their answer back to the parameter server (PS). This sums them and updates the model. By applying \solon{}, we reduce the communication complexity for sending gradients to server from $\mathcal{O}(Pd)$ to $\mathcal{O}(Pd_c)$. The broadcast phase of sending aggregated gradients from server to compute nodes takes $\mathcal{O}(\log{(P)}d)$, which is not the major overhead. 

\eat{
\vspace{0.1in}
\begin{remark}
	Compared to previous works, our analysis and framework are applicable to any distributed algorithm which requires the sum of multiple functions. Notably, 
the framework can be applied to any first-order methods, including gradient descent, SVRG \cite{johnson2013accelerating}, coordinate descent, and projected or accelerated versions of these algorithms. 
	For the sake of simplicity, our discussion in the rest of the paper will focus on mini-batch SGD.
\end{remark}
}
We assume that at most $s$ compute nodes are unreliable, Byzantine, or adversarial, and can send to the PS an arbitrary update. 

We consider the strongest possible adversaries: with infinite computational power, knowing the entire data set, the training algorithm, any defenses present in the system, and able to collaborate.

\subsection{Framework}	\vspace{-0.1in}
\solon{} is defined by the tuple, or \emph{mechanism}, $(\mathbf{A}, E, D)$, where $\mathbf{A}$ is an allocation matrix specifying how to assign gradients to nodes, $E$ are encoding functions determining how each compute node should locally encode its gradients, and $D$ is a decoding function determining how the PS should decode the output of the nodes. As an example, in Figure \ref{fig:RunningExample}(a), $A$ corresponds to the gradient computation assignment of the compute nodes, $E$ corresponds to the summation of the gradients by each node, and $D$ refers to the decoding phase at the PS. 
We generalize the scheme in Figure \ref{fig:RunningExample} to $P$ compute nodes and $B$ gradients. % \scream {should not say data samples, but gradients?}.

{\bf Allocation matrix, $\mathbf{A}$.} 
At each iteration of the training process, we assign the $B$ gradients to the $P$ compute nodes using a $P\times B$ {\it allocation matrix} $\mathbf{A}$, where $\mathbf{A}_{j,k}$ is equal to unity ("1") if node $j$ is assigned to the $k$th gradient ${\bf g}_k$, and zero ("0") otherwise. The support of $\mathbf{A}_{j,\cdot}$, denoted $\supp\left(\mathbf{A}_{j,\cdot}\right)$, is the set of indices of gradients evaluated by the $j$th node. For simplicity, we will assume $B=P$. % throughout the following.
Let $\|\mathbf{A}\|_0$ be to the $L_0$ norm of a matrix, i.e., the number of nonzero entries.
Following \cite{DRACO}, we define the \emph{redundancy ratio} of an allocation as the average number of gradients assigned to each compute node, or equivalently $r\triangleq  \|\mathbf{A}\|_0/P$.

We define the $d \times P$ matrix $\mathbf{G}$ with gradients as its columns: $\mathbf{G} \triangleq [\mathbf{g}_1,\mathbf{g}_2,\cdots, \mathbf{g}_P]$. The $j$th node first picks out its assigned gradients using the allocation matrix $\mathbf{A}$, computing a $d\times P$ gradient matrix $\smash{\mathbf{Y}_j \triangleq \left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}}$. 
The columns of this matrix are $\mathbf{g}_k$ if the $k$th gradient $\mathbf{g}_k$ is allocated to the $j$th compute node, \ie $\mathbf{A}_{j,k} \not = 0$, and zero otherwise.

{\bf Encoding Functions, $E$.} The $j$th compute node is equipped with an encoding function $E_j$ that maps the $d\times P$ matrix $\mathbf{Y}_j$ of its assigned gradients to a $d_c$-dimensional vector.
The $j$th compute node computes and sends $\smash{\mathbf{z}_j \triangleq E_j(\mathbf{Y}_j)}$ to the PS.
If the $j$th node is adversarial, then it instead sends $\smash{\mathbf{z}_j+\mathbf n_{j}}$ to the PS, where $\mathbf n_{j}$ is an arbitrary $d_c$-dimensional \emph{Byzantine} vector.
We let  $E = \{ E_1, E_2, \cdots, E_P\}$ be the set of local encoding functions.

{\bf Decoding Function, $D$}. The $d_c \times P$ matrix $\smash{\mathbf{Z}=\mathbf{Z}^{\mathbf{A},E,\mathbf{G}} \triangleq [\mathbf{z}_1, \mathbf{z}_2,\cdots, \mathbf{z}_P]}$ contains all outputs of the nodes. The $d_c \times P$ matrix $\smash{\mathbf{N} \triangleq [\mathbf{n}_1, \mathbf{n}_2,\cdots, \mathbf{n}_P]}$ contains all Byzantine vectors, with at most $s$ non-zero columns.
Then, the PS receives a $d_c\times P$ matrix $\smash{\mathbf{R} \triangleq \mathbf{Z} +\mathbf{N}}$, and computes a $d$-dimensional vector $\smash{\mathbf{u} \triangleq D(\mathbf{R})}$ using a decoding function $D$.


We require that the algorithm at the PS recovers the $d$-dimensional sum of gradients, $\mathbf{G} \mathbf{1}_P$:

\begin{definition}
	\solon{} with $(\mathbf{A}, E, D)$ can tolerate $s$ adversarial nodes, if for any $\mathbf{N} = [\mathbf{n}_1,\mathbf{n}_2,\cdots, \mathbf{n}_P]$ such that $ \left\vert{ \{j:\mathbf{n}_{j}\not=0\} }\right\vert \leq s$, we have $D(\mathbf{Z}+\mathbf{N}) = \mathbf{G}\mathbf{1}_P$.
\end{definition}

If we defend against the Byzantine attack, then the model update at each iteration is identical to the adversary-free setting. 
This implies that  convergence guarantees for the adversary-free case transfer to the adversarial case.

\subsection{Encoding and decoding functions}	\vspace{-0.1in}
What are the fundamental limits of the above allocation, encoding, and decoding schemes, in particular of the redundancy ratio used in allocation and the compression ratio used in encoding?  Perhaps surprisingly, \emph{the redundancy ratio does not depend on the compression ratio}.
The encoded gradients at each compute node can be arbitrarily compressed without affecting the our ability to tolerate Byzantine attacks.
The reason is that any $d$-dimensional real vector can be mapped one-to-one to a real number. This is stated in the following theorem.

\begin{theorem}\label{Thm:GenericBound}
	If there is a mechanism $(\mathbf{A}, E, D)$ of gradient allocation, encoding, and decoding with redundancy ratio $r$ tolerating $s$ adversarial nodes with a compression ratio $r_c$ of unity, then there is a mechanism $(\mathbf{A}', E', D')$ with redundancy ratio $r$ tolerating $s$ adversarial nodes for any compression ratio $r_c>0$.
\end{theorem}


However $(\mathbf{A}', E', D')$ is in a sense pathological and it is unclear if it can reduce the the number of bits communicated.
Therefore, we seek classes of \textit{regular} encoder and decoder functions $E,D$, to reduce communication cost.

\begin{definition}
	 A set of encoding functions $E$ is called {\em regular} if each output element of each function $E_j$ is a function of linear combinations of columns of the input. Formally, if $E_{j,v}$ is the $v$th element of $E_j$, then
	 $(\mathbf{A}, E, D)$ is regular if there exists a $d\times P$ matrix $\mathbf{U}_{j,v}$ and functions $\smash{\hat{E}_{j,v}}$, such that $\smash{E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}\left(\mathbf{1}_d^T\left(\mathbf{U}_{j,v} \odot \mathbf{Y}_{j}\right)\right)}$.
\end{definition}

%To better understand the \textit{regular} condition, 
When $d=1$, $\mathbf{Y}_j$ has only one row and $\mathbf{1}_{d}=1$ is a scalar.
Thus, $E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}(\mathbf{U}_{j,v} \odot \mathbf{Y}_j)$ implies that $E$ is an arbitrary function of $\mathbf{Y}_j$.
When $d>1$, each output coordinate only depends on linear combinations of input columns.
Since linear combinations do not introduce extra bits, this allows practical communication compression. We will study regular encoders $E$.

\paragraph{Redundancy Bound.}
We first study redundancy requirements for exact recovery of the sum of gradients with $s$ adversaries and compression ratio $r_c$. 
\begin{theorem}\label{Thm:RedundancyRatioBound}
A mechanism $(\mathbf{A}, E, D)$ of gradient allocation, regular encoding, and decoding with compression ratio $r_c$ tolerating $s$ adversarial nodes must have a redundancy ratio $r \geq 2s+r_c$.
\end{theorem}

Thus, for any regular encoder, each gradient has to be replicated on average at least $2s+r_c$ times to defend against $s$ adversarial nodes with a communication compression ratio of $r_c$. If a mechanism tolerates $s$ adversarial nodes with a communication compression ratio of $r_c$, by Theorem \ref{Thm:RedundancyRatioBound}, each compute node encodes at least $(2s+r_c)$ $d$-dimensional vectors on average. If the encoding has linear time complexity, then each encoder requires $O((2s+r_c)d)$ operations in the worst case. If the decoder $D$ has linear time complexity, then it requires at most $O(Pd_c)$ operations in the worst case, as it needs to use the $d$-dimensional input from all $P$ compute nodes. This gives a computational cost of $O(Pd_c)$, which is less than the bound $\mathcal{O}(Pd)$  for the repetition code in \cite{DRACO}.

To better understand the lower bound, we give an equivalent formulation it in the language of linear algebra. Let $g$ be one of the $d\times 1$ dimensional gradients. Suppose it gets sent to $r$ nodes. Then the potentially  corrupted output of the linear encoder at each node $j$  can be represented by $R_j = Z_j g + n_j$, and $n_j$ is the noise here for $j=1,\ldots, r$, where each $Z_j$ is a $d_c \times d$ dimensional matrix. If the number of adversaries is at most $s$, then at most $s$ vectors $n_j$ are nonzero. We call this set of perturbation $B_{s,r}$. Thus, the goal is to design the $r$ matrices $Z_j$, such that for any collection of vectors $n_j$ at most $s$ of which are nonzero, it is possible to recover $g$ from the observations $(Z_j,r_j)$, $j=1,\ldots, r$.
Let $R:=(R_1,\ldots, R_r)$ and $n:=(n_1,\ldots,n_r)$, which we view as a concatenation of vectors belonging to the allowed set $B_{s,r}$. For the recovery of $g$ to be possible, we need that if $R(g,n) = R(g',n')$ for $g,g'\in \R^d$ and $n,n'\in B_{s,r}$, then $g=g'$. 

We can write $R$ as a linear function $R = Zg+n$, where $Z$ is an $rd_c\times d$ concatenation of the matrices $Z_i$. Thus, we can write $R(g,n) = R(g',n')$ as
$Zg+n=Zg'+n' \iff Z(g-g')=n-n'.$
Moreover, we have $n''  = n-n' \in B_{2s,r}$, because at  most $2s$ of its $P$ sub-vectors of size $d_c$ are nonzero. Clearly, all vectors in $B_{2s,r}$ can be written in this form.  Denoting $x = g-g'$, the problem is to understand when there exists a matrix $Z$ such that for all $x \in \R^d$, we have $Zx \notin B_{2s,r}$. Now, $B_{2s,r}$ is a union of several $2sd_c$-dimensional linear subspaces in $rd_c$ dimensions. Moreover, $Zx$ belongs to $span(Z)$, which is an at most $d$-dimensional subspace in $rd_c$ dimensions. Thus, for this to be possible, by counting dimensions we obtain that we need $rd_c\ge 2sd_c +d$. Since $r_c=d/d_c$, this is equivalent to $r\ge 2s +r_c$. This finishes the proof of the fundamental lower bound on the redundancy.



\subsection{Optimal Coding Schemes}
\label{ocs}
%\paragraph{Optimal Coding Schemes}
	\vspace{-0.1in}
Can we achieve the optimal redundancy bound with linear-time encoding and decoding? 
More formally, can we design a tuple $(\mathbf{A},E,D)$ with redundancy ratio $r=2s+r_c$ and computation complexity $\mathcal{O}((2s+r_c)d)$ at the compute nodes and $\mathcal{O}(Pd_c)$ at the PS?
We give a positive answer by designing certain {\em linear block codes} that match the above bounds. 


This is a challenging problem. In fact, we can show (see Appendix \ref{sp}) that this question is \emph{exactly equivalent to a sparse recovery problem}, where we wish to recover an unknown sparse vector from linear combinations of a fixed set of vectors \cite{chen1994basis,chen2001atomic,elad2010sparse}. 
With this lens, our algorithms are related to the classical Prony's method in signal processing \cite{hurst1987scattering,Prony}. However, a key difference is that in our case, we have a \emph{structured set of perturbations}, where entire sub-vectors corresponding to gradients are perturbed at the same time. We leverage this to develop algorithms faster than Prony's method.
\vspace{-0.1in}
\paragraph{Linear Block Code.} 

We focus on the case when $2s+r_c$ divides $P$; otherwise we can change $P$ or $r_c$ until $2s+r_c$ divides $P$. 
Divide the compute nodes into $q:=P/(2s+r_c) = P/r$ ``blocks'' or groups.
We assign each node in the same block to compute the same gradients. 
Each node sends some linear combination of coordinates of the assigned gradients to the PS (``linear'').
The PS solves systems of linear equations to get the desired gradient sum.  
Following the convention of coding theory \cite{abclbc}, we call our approach \textit{linear block codes}.

The linear block code $(\mathbf{A}, E, D)=(\mathbf{A}^{LBC}, E^{LBC}, D^{LBC})$ is defined as follows. 
The assignment matrix is $\mathbf{A} = \mathbf{I}_q \otimes \mathbf{1}_{r \times r}$.

The $j$th compute node first selects its allocated gradients $\mathbf{Y}_j=\left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}$.
Its encoder function sums up the allocated gradients into $\mathbf{Y}_j \mathbf{1}_P$, then computes and sends $\mathbf{z}_j = E_j(\mathbf{Y}_j) = \mathbf{W}_j \mathbf{Y}_j\mathbf{1}_P$  to the PS, where $\mathbf{W}_j$ is a $d_c \times d$ matrix. 
%That is, It then sends $\mathbf{z}_j = E_j^{\mathit{Rep}}(\mathbf{Y}^{Rep}_j)$.

The decoder function, summarized in Algorithm \ref{Alg:DecoderFunction_LinearBlock}, partitions the received updates into the $q$ blocks computing identical gradients.
For each, a block decoder $\psi(\cdot,\cdot)$ is called to recover the sum of all gradients in this group.
\vspace{-0.1in}
\begin{algorithm}[htbp]
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{Received $d_c \times P$ matrix $\mathbf{R}$}
	\Output{Desired gradient summation $\mathbf{u}$}
	Let $\mathbf{R} = \left[\mathbf{R}_1, \mathbf{R}_2, \cdots, \mathbf{R}_{q}\right]$, where each $\mathbf{R}_j$ is a $d_c\times r $ matrix
	
    \For{$j=1$ \KwTo $q$ }
    {
         \textrm{ } $ V = \phi(\mathbf{R}_j,j)$ // Locate the adversarial nodes\\
		$U = \{1,2,\cdots,r\} \setminus V$ // Non-adversarial nodes\\
    $\mathbf{u}_j = \psi(\mathbf{R}_j,j, U)$ // Decode each block using the non-adversarial nodes
    }
	%into $d_c\times r$ matrices
	Compute and return $\mathbf{u} = \sum_{i=1}^{q}\mathbf{u}_i$
	\caption{Decoder Function $D$.}
	\label{Alg:DecoderFunction_LinearBlock}
\end{algorithm}
% \vspace{-0.1in}

There are three questions left: (i) how $\mathbf{W}_j$ is constructed, (ii) how the adversarial node index location function $\phi(\cdot)$ works, and (iii) how the block decoder function $\psi(\cdot,\cdot)$ works.


Given any distinct nonzero scalars $w_1, w_2, \cdots, w_P$, we propose to construct $\mathbf{W}_j$ as $\mathbf{W}_j \triangleq \mathbf{I}_{d_c}\allowbreak$ $\otimes [\allowbreak1,\allowbreak w_j,\allowbreak w_j^2,\allowbreak \cdots,\allowbreak w_j^{r_c-1}]$. The adversarial node index locating function $\phi(\cdot)$ works as follows.
Given the $d_c \times r$ matrix $\mathbf{R}_j$ received from the compute nodes, we first generate a $1\times d_c$ random vector $ \mathbf{f} \sim \mathcal{N}(\mathbf{1}_{1\times d_c},\,\mathbf{I}_{d})$,
and then compute $\smash{\mathbf{r}_{j,c} \triangleq \mathbf{f} \mathbf{R}_j}$.
Next, we obtain an $r$-dimensional vector $\mathbf{a} = [a_1, a_2,\cdots, a_{r}]$ by  solving the linear system
$\begin{bmatrix}
     \hat{\mathbf{W}}_{j,r_c+s-1},\allowbreak  & -\hat{\mathbf{W}}_{j,s-1} \odot\allowbreak \left( \mathbf{r}_{j,c}^T \mathbf{1}_{s}^T\right)
\end{bmatrix}
    \mathbf{a}= \mathbf{r}_{j,c} \odot \left[\hat{\mathbf{W}}_{j,s}\right]_{\cdot,s}$,
 where 
	\[
\hat{\mathbf{W}}_{\mathit{j},v} \triangleq
\begin{bmatrix}
1 & w_{(j-1)r+1} &  w_{(j-1)r+1}^2 &\cdots &  w_{(j-1)r+1}^{v} \\
1 & w_{(j-1)r+2} &  w_{(j-1)r+2}^2 &\cdots &  w_{(j-1)r+2}^{v} \\
\vdots & \vdots & \vdots & \vdots & \vdots\\
1 & w_{jr} &  w_{jr}^2 &\cdots &  w_{jr}^{v}
 \\
\end{bmatrix}.
\\
\]
Finally compute $P_j(w) \triangleq (\sum_{i=0}^{r_c+s-1} a_{i+1} w^i)/(w^s+\sum_{i=0}^{s-1} a_{i+r_c+s+1} w^i) $,
and return $V=\{i|P_j(w_{(r-1)j+i}) \not =\left[ \mathbf{r}_{j,c}\right]_i\}$.
The decoding function $\psi(\cdot, \cdot)$ computes and returns $\textit{vec}\left(\left[\mathbf{R}_{j}\right]_{\cdot, U} \left[\hat{W}_{j,r_c-1}\right]_{U,\cdot}^{-1,T}\right)$ given the non-adversarial node indices $U$.

The following lemma ensures that the Byzantine nodes are correctly found.
\begin{lemma}\label{Thm:LBCDetection}
	Suppose $\left\vert{\{j:\|\mathbf{n}_{j}\|_0 \not=0\}}\right\vert$ $\leq s$ and $r\geq r_c+2s$. 
	Then $\phi(\mathbf{R}_j,j) =  \{i:\|\mathbf{n}_{j(r-1)+i}\|_0 \not=0\}$ with probability equal to unity. 
\end{lemma}
The next lemma demonstrates that within each group the gradient is correctly recovered.
\begin{lemma}\label{thm:LBClocalcorrect}
	If $U$ consists solely of at least $r-s$ non-adversarial nodes, then  with probability equal to unity, $\mathbf{u}_j = \sum_{k=(j-1)r+1}^{jr}\mathbf{y}_{k}$.
\end{lemma}

Combing the above two results,  we show that the linear block code tolerates any $s$ adversaries, achieving the optimal redundancy and compression ratio with linear-time encoding and decoding.

\begin{theorem}\label{Thm:LinearBlockCodeOptimality}
	The linear block code  $(\mathbf{A}, E, D)$ tolerates any $s$ adversaries with probability equal to unity, and achieves the redundancy ratio  bound. For $d\gg P$, its encoding and decoding achieve linear-time computational complexity. 
% \ed{clarify}
\end{theorem} 

Theorem \ref{Thm:LinearBlockCodeOptimality} shows that the linear block code is information theoretically tight and enjoys a small computational overhead even for large ML models. 
 


==> Figure/macros.tex <==
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{amsthm,amsmath,amssymb}
%\usepackage{graphicx,xspace,verbatim,comment}
%\usepackage{array,color,multirow}
%\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{float,url,amsfonts,alltt}
\usepackage{mathtools,rotating}
\usepackage{ifpdf,fancyvrb}
\usepackage{enumitem}
%\usepackage{algorithm,algpseudocode}
%\usepackage{etoolbox,listings,subcaption}
%\usepackage{bigstrut,morefloats}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
%\usepackage{thm-restate}
%\usepackage{todonotes}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
\usepackage{subfigure}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}

\usepackage{graphicx,xspace,verbatim,comment}
\usepackage{hyperref,array,color,balance,multirow}
\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{mathtools,rotating,amsmath,amssymb}
\usepackage{color,ifpdf,fancyvrb,array}
% \usepackage{algorithm,algpseudocode}
\usepackage{etoolbox,listings}
%\usepackage{subcaption}
\usepackage{bigstrut,morefloats}
\usepackage{makecell}
%\usepackage[boxruled]{algorithm2e}
\usepackage{pbox}
\usepackage[numbers]{natbib}
\usepackage{algorithm, algorithmic}
\usepackage[boxruled,algo2e,linesnumbered]{algorithm2e}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newcommand{\eat}[1]{}

\newcommand{\gaussian}[2]{\mathcal{N}(#1,#2)}


% User Defined Commands
\newcommand{\systemnameSolon}{\textsc{Solon}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\cmp}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\detox}{\textsc{Detox}}
\newcommand{\draco}{\textsc{Draco}}
\newcommand{\solon}{\textsc{Solon}}
\newcommand{\bulyan}{\textsc{Bulyan}}
\newcommand{\multikrum}{\textsc{Multi-Krum}}
\newcommand{\signum}{\textsc{Signum}}
% \newcommand{\eg}{\textit{e.g., }}
% \newcommand{\ie}{\textit{i.e., }}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\hier}{\textsc{Hier-Aggr}}
%
\newcommand{\lingjiao}[1]{{\color{blue} {\bf Lingjiao:} #1}}
\newcommand{\leshang}[1]{{\color{red} {\bf Note:} #1}}

\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\indi}{\mathds{1}}
\newcommand{\ie}{{\emph i.e.,} }
\newcommand{\eg}{{\it e.g.}, }
\newcommand{\tr}{\operatorname{tr}}
% \newcommand{\R}{\mathbb{R}}
%\newcommand{\C}{\mathbb{C}}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\cov}{\operatorname{Cov}}
% \newcommand{\PP}{\mathbb{P}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecwb}{\mathbf{w}}
\newcommand{\tvecw}{\widetilde{\mathbf{w}}}
\newcommand{\tvecwb}{\widetilde{\mathbf{w}}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\ovecv}{\overline{\mathbf{v}}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\tvecz}{\widetilde{\mathbf{z}}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\gradf}{\nabla f}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\gradtf}{\nabla \widetilde{f}}
\newcommand{\gradF}{\nabla F}
\newcommand{\HW}{\textsc{Hogwild!}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\const}{\mathcal{O}(1)}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\CM}{\textsc{KroMagnon}}
\newcommand{\cdeg}{\overline{\Delta}}
\newcommand{\ct}{\mathcal{O}(1)}
\newcommand{\W}{\mathcal{W}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norms}[1]{\|#1\|}
\newcommand{\twonm}[1]{\left\|#1\right\|_2}
\newcommand{\twonms}[1]{\|#1\|_2}
\newcommand{\onenm}[1]{\left\|#1\right\|_1}
\newcommand{\onenms}[1]{\|#1\|_1}
\newcommand{\fbnorm}[1]{\left\|#1\right\|_F}
\newcommand{\fbnorms}[1]{\|#1\|_F}
\newcommand{\prob}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\probs}[1]{\mathbb{P}\{#1\}}
\newcommand{\EXP}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\EXPS}[1]{\mathbb{E}[#1]}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\innerp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\innerps}[2]{\langle#1,#2\rangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\abss}[1]{|#1|}
\newcommand{\tsp}{^{\rm T}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\mt}{B\floor{t/B}}
%\newcommand{\G}{\overline{G}}
%\newcommand{\B}{\overline{B}}
\numberwithin{equation}{section}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\red}[1]{{\color{red}{#1}}}

\newcommand{\paris}[1]{{\color{red} #1}}


\newcommand\overmat[2]{%
	\makebox[0pt][l]{$\smash{\color{white}\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{\color{black}#1}}}$}#2}
\newcommand\bovermat[2]{%
	\makebox[0pt][l]{$\smash{\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{#1}}}$}#2}
					
\newcommand\bundermat[2]{%
	\makebox[0pt][l]{$\smash{\underbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}_{\text{#1}}}$}#2}
					
					
\newcommand\partialphantom{\vphantom{\frac{\partial e_{P,M}}{\partial w_{1,1}}}}

\newcommand{\scream}[1]{{\bf * #1 *}{\typeout{#1}}}

\usepackage{amsmath}
\usepackage{accents}
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
    
%\usepackage{algorithm,algpseudocode}


\newtheorem{theo}{Theorem}
\newtheorem{introtheo}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{rem}{Remark}
\newtheorem{asm}{Assumption}
\newtheorem{example}{Example}
\newtheorem{property}{Property}

\newcommand{\blkdiag}{\text{blkdiag}}
\newcommand{\GGG}{{\color{red}{\bf [GGG CHECK]}}}
\newcommand{\sort}{\text{sort}}
\newcommand{\Span}{\text{span}}
\newcommand{\supp}{\text{supp}}
\newcommand{\bsp}{\hspace{-0.14cm}}
\newcommand{\T}{\intercal}
\newcommand{\eqdef}{\stackrel{\triangle}{=}}
\newcommand{\G}{ \mathcal{G} } 
\newcommand{\Gnp}{ \mathcal{G}\left(n,\frac{1}{2}\right) } 
\newcommand{\Gnpk}{ {G}\left(n,\frac{1}{2}, k\right) }
\newcommand{\opt}{\textsf{opt}}
\newcommand{\A}{{\bf A}}
\newcommand{\den}{\textsf{den}}
\usepackage[T1]{fontenc}
\usepackage{upgreek}

\newcommand{\Exp}{\mathbb{E}}
\usepackage[greek,english]{babel}
% \usepackage[utf8x]{inputenc}
\usepackage{pifont}
\usepackage{float}
\usepackage{autobreak}


==> Solon_Arxiv (5)/Conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}\label{Sec:SOLON:Conclusion}
\vspace{-0.1in}

In this paper, we propose \systemnameSolon{}, 
a distributed training framework that simultaneously resists Byzantine attack and reduces communication overhead via algorithmic redundancy. 
We show that there is a fundamental trade-off between Byzantine-resilience, communication cost, and computational cost.
Extensive experiments show that \solon{} provides significant speedups over existing methods, and consistently leads to successful convergence under different attacks. 

==> Solon_Arxiv (5)/Experiment.tex <==
\vspace{-0.1in}
\section{Experiments}\label{Sec:SOLON:Experiment}
\vspace{-0.1in}
Now we present an empirical study on \solon{} compared with several existing methods including \draco{}~\cite{DRACO}, \bulyan{}~\cite{guerraoui2018hidden}, and \signum{}~\cite{bernstein2018signsgd}. 
Across diverse ML models trained on real world datasets, we have found 1) that \solon{} results in significant speedups over existing methods, including $10\times$ faster than \bulyan{} and $80\%$ faster than \draco{} while reaching the same accuracy, and  2) that \solon{} consistently leads to successful convergence for all Byzantine attacks considered, while previous approaches may fail on different attacks (\eg \signum{} on constant attack, and \bulyan{} on "A little is enough" (ALIE) attack~\cite{ALIE2019}). 

\begin{table}[b]
\centering
\begin{minipage}{.58\linewidth}
    \medskip
    % \raggedleft
	\centering
	\caption{Summary of the datasets, models, and hyper-parameters used in our experiments.}
	\scalebox{0.95}{
	\begin{tabular}{cccc}
		\toprule Dataset
		& CIFAR-10 & SVHN & \makecell{WikiText-2}\bigstrut\\
		\midrule
		\midrule
		\# data points & 60,000 & 600,000 & 2,551,843 \bigstrut\\
		Model & ResNet-18 & VGG13-BN  & LSTM \bigstrut\\
		\# Parameters & 11,173k & 9,923k  & 7,332k \bigstrut\\
		Optimizer & SGD & SGD &SGD \bigstrut\\
		Batch Size & 120 & 120 & 60 \bigstrut\\
		\bottomrule
    	\end{tabular}
    	}%
    % 	\vspace{-2mm}
		\label{Tab:solon:DataStat}%
\end{minipage}
\hskip 10pt
% \hfill
\begin{minipage}{.37\linewidth}
% \raggedright
    \medskip
	\centering
% 	\vspace{0.3 cm}
    \caption{The size of gradients to transmit per worker before and after compression (MB, $10^6$ bytes). }
    \scalebox{0.86}{
	
	\begin{tabular}{cccc}
		\toprule Model & 
		  ResNet18 & VGG13 & LSTM \bigstrut\\
		\midrule
		\midrule
		Size & 89.6 & 79.4 & 58.8   \bigstrut\\
% 		$r_c=4$ & 22.4 & 19.84 & 34.4 \bigstrut\\
		$r_c=6$ & 14.9 & 13.2 & 9.78 \bigstrut\\
		$r_c=8$ & 11.2 & 9.92 & 7.35  \bigstrut\\
		$r_c=10$ & 8.96  & 7.94  & 5.88  \bigstrut\\
		
		\bottomrule
	\end{tabular}
	}%
% 	\vspace{-3mm}
	\label{Tab:compressionsize}
	\end{minipage}
	\vspace{-3mm}
\end{table}

\begin{figure}[t] 
\centering
\includegraphics[width=0.94\textwidth]{Figure/accu_iter_hour_legend_node50.pdf}\\
\vspace{-2mm}
\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_iter_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps,  constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_ALIE_node50_ResNet.pdf}}\\
\vspace{-3mm}
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_ALIE_node50_ResNet.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} and other baselines on ResNet-18 and CIFAR-10. (a)-(c): Comparison of test accuracy vs. the number of iterations between 
\solon{} $r_c=10$ and other methods under different attacks. (d)-(f): Test accuracy vs. running time of \solon{} and other methods. Vanilla SGD simply averages gradients received on PS and is tested without adversary. Accuracy may fluctuate occasionally due to randomness and lr adjustments.} }
\vspace{-5mm}
\label{fig:against-defense}
\end{figure}

\paragraph{Experimental setup.} 
We implement \solon{} in PyTorch~\cite{paszke2019pytorch} with MPI~\cite{DALCIN20051108}.
The experiments were conducted on a cluster of 50 real machines from Cloudlab  \cite{CloudlabDuplyakin} with 1 Gbps network speed and 100 virtual compute nodes. We trained three large scale models, namely, ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10}, VGG13-BN~\cite{VGGverydeepconv} on SVHN~\cite{svhn}, and a two-layer stacked LSTM \cite{LSTMnips96} (nhid=200) on WikiText-2~\cite{wikitext-2}, respectively.  
The details are summarized in Table \ref{Tab:solon:DataStat}.
For comparison with \solon{}, we also evaluate two robust aggregator-based approches, \bulyan{}, \signum{}, and an algorithmic redundancy-based approach, \draco{}.  \solon{} splits the virtual machines evenly into 5 groups, each with 20 redundant machines. To compare with the best possible performance of \draco{}, we set the $r=11$ and only use 5 groups for \draco{} to reduce its communication overhead. 
More details are in the appendix.

\vspace{-2mm}
\paragraph{Attacks.} We use three different attacks:  reverse gradient,  constant, and ALIE (``A little is enough''~\cite{ALIE2019}). 
In the reverse gradient attack (rev-grad), Byzantine nodes always send $\kappa$ times the true gradient to the PS. 
In the constant attack, Byzantine nodes always send a constant multiple $c$ of the all-ones vector.
In the experiments shown, $\kappa = -100$ and $c=-100$.

In ALIE, Byzantine nodes use local information to estimate the mean and variance of the gradients computed at the other nodes, and then manipulate the gradient as $ \hat{\mu} + z \cdot \hat{\sigma}$ where $\hat{\mu}$ and $\hat{\sigma}$ are the mean and standard deviation of the gradients estimated by Byzantine nodes and $z$ is an adjustable hyper-parameter that adds an unnoticeable perturbation to disrupt the aggregation. In experiments, we set $z=1$.   
% \lingjiao{explain value of $z$}
At each iteration, we randomly select $s = 5$ compute nodes as adversaries. 

% \subsection{Results} 
% \label{subsec:result}
\vspace{-2mm}
\paragraph{End to end performance.} We start by evaluating \solon{}'s end to end performance along with the baseline methods under different attacks, which is shown in Figure~\ref{fig:against-defense}.
We first note that previous approaches may result in significant accuracy loss under certain attacks. For example, \signum{}'s accuracy is 30\% worse than   the Byzantine-free vanilla SGD under constant attack (Figure~\ref{fig:against-defense}(b)), and ALIE attack leads a 50\% accuracy drops for \bulyan{} (Figure~\ref{fig:against-defense}(c)).
Nevertheless, across different attacks, \solon{} consistently converges and matches the accuracy performance of the vanilla SGD in a Byzantine-free environment. 
This is primarily due to \solon{}'s black box performance guarantee.

\begin{figure}[t]
\vspace{-4mm}
\centering
\subfigure[ResNet18, CIFAR-10]{\includegraphics[width=0.33\textwidth]{Figure/time_breakdown_4methods_RN18_node50.pdf}}
\subfigure[VGG13-BN, SVHN ]{\includegraphics[width=0.31\textwidth]{Figure/time_breakdown_4methods_node50_SVHN_revgrad.pdf}}
\subfigure[LSTM, WikiText-2]{\includegraphics[width=0.30\textwidth]{Figure/time_breakdown_4methods_RN18_node50_LSTM.pdf}}
\vspace{-3mm}
\caption{\footnotesize{Time breakdown per iteration of \solon{} $r_c=10$ and all baseline methods over three models+datasets under rev-grad. The types of attack will not affect most of the times. Notice that even if \signum{} is the fastest in time per iteration among those methods, and even faster than vanilla SGD, its accuracy is sacrificed and thus \solon{} still has the best convergence performance.}} 
\label{fig:timebreakdown}
\vspace{-5mm}
\end{figure}
% \vspace{-4mm}

\begin{figure}[t]
  \centering
  \subfigure[Speed up ($\times$) of \solon{}]{\includegraphics[width=0.42\textwidth]{Figure/solon_speedup_heatmap_node50_RN18.pdf}}
  \hskip 20pt
  \subfigure[Time breakdown of \solon{}]{\includegraphics[width=0.40\textwidth]{Figure/time_breakdown_solonrc_node50_RN18_fixn.pdf}}
  \vspace{-3mm}
  \caption{\footnotesize{(a) The speed up ($\times$) of \solon{}, $r_c=10$ vs other baselines on converging to certain test accuracy level on ResNet-18+CIFAR-10 under selected attacks. Values are approximation. $\infty$ means the method does not converge to the accuracy in the experiment. (b) Time breakdown of \solon{} by varying $r_c$, fixing $s$ with similar \# of compute nodes on ResNet-18 trained over the CIFAR-10 dataset (regardless of attacks). } }
  \vspace{-3mm}
  \label{fig:solonspeedup}
\end{figure}

\begin{figure}[ht] 
\centering
\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_iter_3000_revgrad_node50_LSTM.pdf}}
\hskip 20pt
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_hour_3000_revgrad_node50_LSTM.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} $r_c=10$ and other baselines on LSTM model trained over WikiText-2 dataset under reverse gradient attack, $s=5$. (a) Validation perplexity vs. \# iterations. (b) Validation perplexity vs. running time. }}
\label{fig:against-defense:appendix:LSTM}
\vspace{-3mm}
\end{figure}

Furthermore, \solon{} provides significant runtime speedups over existing methods.
For example, as shown in Figure \ref{fig:against-defense}(d), \solon{} converges faster than all the other Byzantine-resilient approaches. 
Its runtime performance even outperforms the vanilla SGD in a Byzantine-free environment.
This is primarily due to the communication efficiency of \solon{}. We observe a similar trend for the other two models (\eg LSTM under rev-grad attack shown in Figure \ref{fig:against-defense:appendix:LSTM}). 
Figure \ref{fig:solonspeedup}(a) gives a quantitative result of the speedups achieved by \solon{}.
To achieve a 90\% test accuracy, \solon{} obtains a speedup of 1.8$\times$ over \draco{} and 11$\times$ over \bulyan{} under the reverse gradient attack, while  \signum{} cannot reach 90\% accuracy. Other details and results can be found in the Appendix. 

\vspace{-2mm}
\paragraph{Per iteration cost.} 
Next, we dive into the per iteration cost of each approach.
As shown in Figure \ref{fig:timebreakdown}.
We note that \bulyan{} requires a significantly higher decoding time than all the other methods. 
This is probably because \bulyan{} deploys a computational expensive robust aggregator. 
Note that \solon{} reduces the communication cost by slightly increasing the computation and decoding complexity compared to \draco{}. Nevertheless, across all datasets and models considered in our experiments, \solon{} attains the fastest per iteration runtime.
This is because \solon{} largely reduces the communication cost, which is the bottleneck in a large cluster, and the extra computation and decoding cost is relatively small. 

\vspace{-2mm}
\paragraph{Effects of compression ratio.}
Finally we evaluate the effects of the compression ratio $r_c$ on \solon{}'s performance, as shown in Figure \ref{fig:solonspeedup}(b).
Here we vary compression rate $r_c$, fix attacks $s$, and change redundancy ratio $r$ accordingly. We keep the entire number of machines roughly at the same level by varying group numbers. 
Overall, as the compression ratio decreases, the communication cost increases almost linearly, and thus the total runtime.
This shows that \solon{} can be applied for different communication requirements with small extra overhead. 
In addition, we observe that the computation cost increases slightly when $r_c$ goes up, since the increase of $r_c$ will require an increase in the group batch size. The decode time also changes slightly. However, these are not major factors compared to communication. 
Other details can be found in the appendix.

In addition, we also evaluate the size of the gradients before and after compression, summarized in Table \ref{Tab:compressionsize}. 
Overall, \solon{} largely reduces the gradient size up to 10$\times$, depending on the specified compression ratio $r_c$.
In fact, \solon{} allows users to specify the compression ratio explicitly to satisfy different clusters' requirements. 


==> Solon_Arxiv (5)/Figure/Conclusion.tex <==
\vspace{-0.1in}
\section{Conclusion}\label{Sec:SOLON:Conclusion}
\vspace{-0.1in}

In this paper, we propose \systemnameSolon{}, %\footnote{Our code and data will be available at \url{https://github.com/chenleshang/solon}}
a distributed training framework that simultaneously resists Byzantine attack and reduces communication overhead via algorithmic redundancy. 
We show that there is a fundamental trade-off between Byzantine-resilience, communication cost, and computational cost.
% In addition, \solon{ } utilizes a Vandermonde matrix-based  technique which achieves this trade-off.
Extensive experiments show that \solon{} provides significant speedups over existing methods, and consistently leads to successful convergence under different attacks. 

==> Solon_Arxiv (5)/Figure/Experiment.tex <==
\vspace{-0.1in}
\section{Experiments}\label{Sec:SOLON:Experiment}
\vspace{-0.1in}
Now we present an empirical study on \solon{} compared with several existing methods including \draco{}~\cite{DRACO}, \bulyan{}~\cite{guerraoui2018hidden}, and \signum{}~\cite{bernstein2018signsgd}. 
Across diverse ML models trained on real world datasets, we have found 1) that \solon{} results in significant speedups over existing methods, including $10\times$ faster than \bulyan{} and $80\%$ faster than \draco{} while reaching the same accuracy, and  2) that \solon{} consistently leads to successful convergence for all Byzantine attacks considered, while previous approaches may fail on different attacks (\eg \signum{} on constant attack, and \bulyan{} on "A little is enough" (ALIE) attack~\cite{ALIE2019}). 

\begin{table}[b]
\centering
\begin{minipage}{.58\linewidth}
    \medskip
    % \raggedleft
	\centering
	\caption{Summary of the datasets, models, and hyper-parameters used in our experiments.}
	\scalebox{0.95}{
	\begin{tabular}{cccc}
		\toprule Dataset
		& CIFAR-10 & SVHN & \makecell{WikiText-2}\bigstrut\\
		\midrule
		\midrule
		\# data points & 60,000 & 600,000 & 2,551,843 \bigstrut\\
		Model & ResNet-18 & VGG13-BN  & LSTM \bigstrut\\
% 		\# Classes & 10 & 10 & 10 \bigstrut\\
		\# Parameters & 11,173k & 9,923k  & 7,332k \bigstrut\\
		Optimizer & SGD & SGD &SGD \bigstrut\\
		%Learning Rate & 0.1 & 0.1 \bigstrut\\
		%Momentum & 0.9 & 0.9 \bigstrut\\
		%\signum{} LR & 5E-5 & 5E-5\bigstrut \\
		Batch Size & 120 & 120 & 60 \bigstrut\\
		\bottomrule
    	\end{tabular}
    	}%
    % 	\vspace{-2mm}
		\label{Tab:solon:DataStat}%
\end{minipage}
\hskip 10pt
% \hfill
\begin{minipage}{.37\linewidth}
% \raggedright
    \medskip
	\centering
% 	\vspace{0.3 cm}
    \caption{The size of gradients to transmit per worker before and after compression (MB, $10^6$ bytes). }
    \scalebox{0.86}{
	
	\begin{tabular}{cccc}
		\toprule Model & 
		  ResNet18 & VGG13 & LSTM \bigstrut\\
		\midrule
		\midrule
		Size & 89.6 & 79.4 & 58.8   \bigstrut\\
% 		$r_c=4$ & 22.4 & 19.84 & 34.4 \bigstrut\\
		$r_c=6$ & 14.9 & 13.2 & 9.78 \bigstrut\\
		$r_c=8$ & 11.2 & 9.92 & 7.35  \bigstrut\\
		$r_c=10$ & 8.96  & 7.94  & 5.88  \bigstrut\\
		
		\bottomrule
	\end{tabular}
	}%
% 	\vspace{-3mm}
	\label{Tab:compressionsize}
	\end{minipage}
	\vspace{-3mm}
\end{table}

\begin{figure}[t] 
\centering
\includegraphics[width=0.94\textwidth]{Figure/accu_iter_hour_legend_node50.pdf}\\
\vspace{-2mm}
\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_iter_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps,  constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs steps, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_iter_3000_ALIE_node50_ResNet.pdf}}\\
\vspace{-3mm}
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.325\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, constant]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_const_node50_ResNet.pdf}}
\subfigure[Accuracy vs time, ALIE]{\includegraphics[width=0.31\textwidth]{Figure/accu_hour_3000_ALIE_node50_ResNet.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} and other baselines on ResNet-18 and CIFAR-10. (a)-(c): Comparison of test accuracy vs. the number of iterations between 
\solon{} $r_c=10$ and other methods under different attacks. (d)-(f): Test accuracy vs. running time of \solon{} and other methods. Vanilla SGD simply averages gradients received on PS and is tested without adversary. Accuracy may fluctuate occasionally due to randomness and lr adjustments.} }

\vspace{-5mm}
\label{fig:against-defense}
\end{figure}


\paragraph{Experimental setup.} 
We implement \solon{} in PyTorch~\cite{paszke2019pytorch} with MPI~\cite{DALCIN20051108}.
The experiments were conducted on a cluster of 50 real machines from Cloudlab  \cite{CloudlabDuplyakin} with 1 Gbps network speed and 100 virtual compute nodes. We trained three large scale models, namely, ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10}, VGG13-BN~\cite{VGGverydeepconv} on SVHN~\cite{svhn}, and a two-layer stacked LSTM \cite{LSTMnips96} (nhid=200) on WikiText-2~\cite{wikitext-2}, respectively.  %and WRN-22-8~\cite{WRNwiderangenet} on on Fashion-MNIST~\cite{fashionmnist}, respectively. 
The details are summarized in Table \ref{Tab:solon:DataStat}.
For comparison with \solon{}, we also evaluate two robust aggregator-based approches, \bulyan{}, \signum{}, and an algorithmic redundancy-based approach, \draco{}.  \solon{} splits the virtual machines evenly into 5 groups, each with 20 redundant machines. To compare with the best possible performance of \draco{}, we set the $r=11$ and only use 5 groups for \draco{} to reduce its communication overhead. 
More details are in the appendix.


\vspace{-2mm}
\paragraph{Attacks.} We use three different attacks:  reverse gradient,  constant, and ALIE (``A little is enough''~\cite{ALIE2019}). 
In the reverse gradient attack (rev-grad), Byzantine nodes always send $\kappa$ times the true gradient to the PS. 
In the constant attack, Byzantine nodes always send a constant multiple $c$ of the all-ones vector.
In the experiments shown, $\kappa = -100$ and $c=-100$.
%Since \signum{} is generally resilient to  flip sign attacks like rev-grad. 
%We set $\kappa = -100$ for the rev-grad attack and $c=-100$ for constant attack. 
In ALIE, Byzantine nodes use local information to estimate the mean and variance of the gradients computed at the other nodes, and then manipulate the gradient as $ \hat{\mu} + z \cdot \hat{\sigma}$ where $\hat{\mu}$ and $\hat{\sigma}$ are the mean and standard deviation of the gradients estimated by Byzantine nodes and $z$ is an adjustable hyper-parameter that adds an unnoticeable perturbation to disrupt the aggregation. In experiments, we set $z=1$.   
At each iteration, we randomly select $s = 5$ compute nodes as adversaries. 


\vspace{-2mm}
\paragraph{End to end performance.} We start by evaluating \solon{}'s end to end performance along with the baseline methods under different attacks, which is shown in Figure~\ref{fig:against-defense}.
We first note that previous approaches may result in significant accuracy loss under certain attacks. For example, \signum{}'s accuracy is 30\% worse than   the Byzantine-free vanilla SGD under constant attack (Figure~\ref{fig:against-defense}(b)), and ALIE attack leads a 50\% accuracy drops for \bulyan{} (Figure~\ref{fig:against-defense}(c)).
Nevertheless, across different attacks, \solon{} consistently converges and matches the accuracy performance of the vanilla SGD in a Byzantine-free environment. 
This is primarily due to \solon{}'s black box performance guarantee.



\begin{figure}[t]
\vspace{-4mm}
\centering

\subfigure[ResNet18, CIFAR-10]{\includegraphics[width=0.33\textwidth]{Figure/time_breakdown_4methods_RN18_node50.pdf}}
\subfigure[VGG13-BN, SVHN ]{\includegraphics[width=0.31\textwidth]{Figure/time_breakdown_4methods_node50_SVHN_revgrad.pdf}}
\subfigure[LSTM, WikiText-2]{\includegraphics[width=0.30\textwidth]{Figure/time_breakdown_4methods_RN18_node50_LSTM.pdf}}

\vspace{-3mm}
\caption{\footnotesize{Time breakdown per iteration of \solon{} $r_c=10$ and all baseline methods over three models+datasets under rev-grad. The types of attack will not affect most of the times. Notice that even if \signum{} is the fastest in time per iteration among those methods, and even faster than vanilla SGD, its accuracy is sacrificed and thus \solon{} still has the best convergence performance.}} 
\label{fig:timebreakdown}
\vspace{-5mm}
\end{figure}

\begin{figure}[t]
  \centering
  \subfigure[Speed up ($\times$) of \solon{}]{\includegraphics[width=0.42\textwidth]{Figure/solon_speedup_heatmap_node50_RN18.pdf}}
  \hskip 20pt
  \subfigure[Time breakdown of \solon{}]{\includegraphics[width=0.40\textwidth]{Figure/time_breakdown_solonrc_node50_RN18_fixn.pdf}}
  \vspace{-3mm}
  \caption{\footnotesize{(a) The speed up ($\times$) of \solon{}, $r_c=10$ vs other baselines on converging to certain test accuracy level on ResNet-18+CIFAR-10 under selected attacks. Values are approximation. $\infty$ means the method does not converge to the accuracy in the experiment. (b) Time breakdown of \solon{} by varying $r_c$, fixing $s$ with similar \# of compute nodes on ResNet-18 trained over the CIFAR-10 dataset (regardless of attacks). } }
  \vspace{-3mm}
  \label{fig:solonspeedup}
\end{figure}

\begin{figure}[ht] 
\centering

\subfigure[Accuracy vs steps, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_iter_3000_revgrad_node50_LSTM.pdf}}
\hskip 20pt
\subfigure[Accuracy vs time, rev-grad]{\includegraphics[width=0.4\textwidth]{Figure/accu_hour_3000_revgrad_node50_LSTM.pdf}}
\vspace{-3mm}
\caption{\footnotesize{End to end convergence performance of \solon{} $r_c=10$ and other baselines on LSTM model trained over WikiText-2 dataset under reverse gradient attack, $s=5$. (a) Validation perplexity vs. \# iterations. (b) Validation perplexity vs. running time. }}
\label{fig:against-defense:appendix:LSTM}
\vspace{-3mm}
\end{figure}

Furthermore, \solon{} provides significant runtime speedups over existing methods.
For example, as shown in Figure \ref{fig:against-defense}(d), \solon{} converges faster than all the other Byzantine-resilient approaches. 
Its runtime performance even outperforms the vanilla SGD in a Byzantine-free environment.
This is primarily due to the communication efficiency of \solon{}. We observe a similar trend for the other two models (\eg LSTM under rev-grad attack shown in Figure \ref{fig:against-defense:appendix:LSTM}). 
Figure \ref{fig:solonspeedup}(a) gives a quantitative result of the speedups achieved by \solon{}.
To achieve a 90\% test accuracy, \solon{} obtains a speedup of 1.8$\times$ over \draco{} and 11$\times$ over \bulyan{} under the reverse gradient attack, while  \signum{} cannot reach 90\% accuracy. Other details and results can be found in the Appendix. 

\vspace{-2mm}
\paragraph{Per iteration cost.} 
Next, we dive into the per iteration cost of each approach.
As shown in Figure \ref{fig:timebreakdown}.
We note that \bulyan{} requires a significantly higher decoding time than all the other methods. 
This is probably because \bulyan{} deploys a computational expensive robust aggregator. 
Note that \solon{} reduces the communication cost by slightly increasing the computation and decoding complexity compared to \draco{}. Nevertheless, across all datasets and models considered in our experiments, \solon{} attains the fastest per iteration runtime.
This is because \solon{} largely reduces the communication cost, which is the bottleneck in a large cluster, and the extra computation and decoding cost is relatively small. 
\vspace{-2mm}
\paragraph{Effects of compression ratio.}
Finally we evaluate the effects of the compression ratio $r_c$ on \solon{}'s performance, as shown in Figure \ref{fig:solonspeedup}(b).
Here we vary compression rate $r_c$, fix attacks $s$, and change redundancy ratio $r$ accordingly. We keep the entire number of machines roughly at the same level by varying group numbers. 
Overall, as the compression ratio decreases, the communication cost increases almost linearly, and thus the total runtime.
This shows that \solon{} can be applied for different communication requirements with small extra overhead. 
In addition, we observe that the computation cost increases slightly when $r_c$ goes up, since the increase of $r_c$ will require an increase in the group batch size. The decode time also changes slightly. However, these are not major factors compared to communication. 

Other details can be found in the appendix.

In addition, we also evaluate the size of the gradients before and after compression, summarized in Table \ref{Tab:compressionsize}. 
Overall, \solon{} largely reduces the gradient size up to 10$\times$, depending on the specified compression ratio $r_c$.
In fact, \solon{} allows users to specify the compression ratio explicitly to satisfy different clusters' requirements. 


==> Solon_Arxiv (5)/Figure/Introduction.tex <==
\section{Introduction}\label{Sec:SOLON:Intro}
%TODO
The growing size of datasets and machine learning models has led to many developments in distributed training using stochastic optimization~\cite{devlin2018bert,deng2009imagenet,sergeev2018horovod,dean2012large,dobriban2020wonder}.
One of the most widely used %distributed training
settings is the {\em parameter server (PS) model}~\cite{li2013parameter,li2014scaling,jiang2020unified}, 

where the gradient computation is partitioned among all compute nodes, typically using stochastic gradient descent (SGD) or its variants. A central parameter server then aggregates the calculated gradients from all compute nodes to update the global model. 


However, scaling PS models to large clusters introduces two challenges: guarding against \textit{Byzantine attacks} and managing  \textit{communication overhead}.
Byzantine attacks include erroneous gradients sent from unreliable compute nodes due to power outages, hardware or software errors, as well as malicious attacks. 
The communication overhead of sending gradients to the PS in large clusters can also be extremely high, potentially dominating the training time, ~\cite{dean2012large,alistarh2017qsgd,wen2017terngrad,Wang18Atomo, DRACO}, since the number of gradients sent is linear in the number of compute nodes. 
Although recent work has studied the problem of
%extensively studied how to protect against 
Byzantine attacks under the PS model~\cite{ALIE2019,guerraoui2018hidden,xie2020fall}, the communication overhead remains prohibitive. For example, ~\cite{blanchard2017machine,chen2017distributed,yin2018byzantine,AggregathorDamaskinosEGGR19} use {\em robust aggregators} at the PS to mitigate  unreliable gradients, 
while ~\cite{DRACO} introduces {\em algorithmic redundancy} to detect and remove Byzantine nodes. 
Robust aggregators are computationally
expensive due to their super-linear  (often quadratic) dependence on the number
of nodes. They also often have limited convergence guarantees under
Byzantine attacks, e.g., only establishing convergence in the limit, or only guaranteeing that the output of the aggregator has a positive inner product with the true gradient. 
They often require strong bounds on the dimension of the model.
Although algorithmic redundancy or coding-theoretic~\cite{Gradient_Coding, DRACO}
approaches offer strong convergence guarantees, these approaches have high communication overhead.

Thus, it remains an open question to simultaneously provide \textbf{\emph{Byzantine-resilience with strong guarantees and communication efficiency}} for distributed learning.





\begin{figure*}[t] 
\centering
\subfigure[Example of a \solon{} instance]{\includegraphics[width=0.6\textwidth]{Figure/intro_fig_2.pdf}}
% \hfill
\hskip 5pt
\subfigure[Performance of \solon{}]{\includegraphics[width=0.37\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet_w_errorbar.pdf}}
\vspace{-2mm}
\caption{\footnotesize{Demonstration of \solon{}. (a) gives an example of \solon{}, where the cluster consists of  four compute nodes.  (b) shows the runtime performance of \solon{} $r_c=10$ when training ResNet-18 on CIFAR-10 under rev-grad attack. Compared to various baselines, \solon{} converges faster and provides higher final accuracy.}}
\label{fig:RunningExample}
% \vspace{-2mm}
\end{figure*}

To address this problem, we propose \solon{}, a distributed training framework leveraging algorithmic redundancy to protect against Byzantine attacks, and ideas from sparse recovery~\cite{Prony} and coding theory~\cite{Gradient_Coding} to reduce communication overhead. 

The approach is as follows: 
In a Byzantine-free PS model with $P$ compute nodes and $B$ gradients to be computed, at each iteration
each of the $P$ nodes computes $B/P$ gradients, and sends them to the PS.  In \solon{}, gradients are computed redundantly to tolerate Byzantine failures; each node computes $rB/P$ gradients, incurring a {\em computational redundancy ratio} of $r$.  To reduce communication overhead, compressed gradients are sent to the PS.  For $d$-dimensional gradients, each node only sends a $d/r_c$-dimensional vector to the PS, where  $r_c$ is the {\em compression ratio}. 

We show that under worst-case adversarial conditions where the adversarial nodes have access to the complete data and gradients, and can send arbitrary results to the PS, there is a fundamental trade-off among Byzantine-resilience, communication overhead and computation cost. To tolerate $s$ Byzantine nodes, the redundancy ratio must satisfy $r\geq 2s+r_c$.
We provide a concrete encoding and decoding technique for \solon{} based on Vandermonde matrices and building on Prony's method from signal processing ~\cite{Prony,communciation_gradcoding_min_ye} that matches the optimal condition  $r= 2s+r_c$. 


\paragraph{Example.}
Figure \ref{fig:RunningExample}(a) shows
four two-dimensional gradient vectors, $g_1, g_2,g_3, g_4$, where gradients $g_i=(g_{i1},g_{i2})$ are in different colors.
To tolerate Byzantine workers, 
%\solon{} requires each compute node to compute redundant gradients. In Figure \ref{fig:RunningExample}(a), 
each node computes four gradients. 
However, instead of sending a two-dimensional vector to the PS, each node only sends a one-dimensional linear combination of the elements in the local gradients. For instance, worker 1 computes and sends the scalar $g_{11}+g_{12}+g_{21}+g_{32}+g_{41}+g_{42}$. Here, the redundancy ratio $r=4$ and the compression ratio $r_c=2$. The PS uses a decoding scheme presented in Section \ref{sec:solon}. Therefore \solon{} can recover the correct gradient with one Byzantine worker ($4 \geq 2\times 1 + 2$). 
\qed


We implemented \solon{} in Pytorch and conducted extensive experiments on a large cluster.  Our results show that
\solon{} can provide significant speedups across various ML models and datasets over existing methods, such as \bulyan{} \cite{guerraoui2018hidden} and \draco{}~\cite{DRACO}, shown in Figure \ref{fig:RunningExample}(b) using ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10} under a reverse gradient attack. 
In addition, 
\solon{} successfully defends against strong Byzantine attacks such as ``A little is enough'' (ALIE)~\cite{ALIE2019}, on which some methods such as \bulyan{} and \signum{} \cite{bernstein2018signsgd} fail to converge or result in significant accuracy loss, see Section \ref{Sec:SOLON:Experiment}. 


\vspace{-0.1in}
\paragraph{Contributions.}   Our contributions include:
\vspace{-0.1in}
\begin{enumerate}
    \item \solon{}, a distributed training framework that exploits algorithmic redundancy to simultaneously provide Byzantine-resilience and communication efficiency. 
    \vspace{-0.07in}
    \item Optimal trade-offs between Byzantine resilience, communication overhead, and computational cost. 
    \vspace{-0.07in}
    \item A concrete encoding and decoding mechanism, which is provably efficient and  achieves this optimal trade-off.
    \vspace{-0.07in}
    \item Extensive experiments which show that \solon{} exhibits significant speedups as well as strong Byzantine-resilience over previous approaches.   
\end{enumerate}

The \solon{} framework can be used for any distributed algorithm which requires the sum of multiple functions, including gradient descent, SVRG \cite{johnson2013accelerating}, coordinate descent, and projected or accelerated versions of these algorithms. However, in this paper, we focus on mini-batch SGD.
The rest of the paper is organized as follows: Section \ref{Sec:SOLON:relatedwork} discusses related work. %, and Section 
Section \ref{sec:solon} presents the \solon{} framework and theoretical guarantees. Experimental results are given in Section \ref{Sec:SOLON:Experiment}. 


\section{Related work}
\label{Sec:SOLON:relatedwork}
Byzantine fault tolerance against worst-case and/or adversarial failures such as system crashes, power outages, software bugs, and adversarial agents that exploit security flaws has been extensively studied since the 1980s~\cite{lamport2019byzantine}. In distributed machine learning, these failures may appear when a subset of compute nodes returns to the PS erroneous updates. It is well understood that first-order methods, such
as gradient descent or mini-batch SGD, are not robust to Byzantine errors; even a single erroneous update can introduce arbitrary errors to the optimization variables~\cite{blanchard2017machine,chen2017distributed}. At the same time, distributed model training suffers from communication overhead due to frequent gradient updates transmitted between compute nodes~\cite{LargeScaleDeepNet_Dean12,mcmahan2017communication,li2014communication,konevcny2016federated,dobriban2020wonder,dobriban2021distributed}. \solon{} aims at improving both Byzantine-resilience and communication-efficiency in distributed model training.

More recently, attention has turned to Byzantine-resilient distributed machine learning techniques.  Results show that while average-based gradient methods are susceptible to adversarial nodes, robust gradient aggregation methods can, in some cases, achieve better convergence while being robust to some attacks~\cite{chen2017distributed,el2019sgd,blanchard2017machine,xie2018zeno,xie2020fall,blanchard2017machine,yin2018byzantine,guerraoui2018hidden,jaggilearningfromhistory}. Despite
theoretical guarantees, the proposed algorithms often only ensure
a weak form of resilience against Byzantine failures, and can fail against strong Byzantine attacks~\cite{guerraoui2018hidden,xie2020fall,ALIE2019}. Another line of work proposes to use algorithmic redundancy to attain black-box Byzantine-resilience guarantees. However, many of these techniques require redundant computation from compute nodes (such as \draco{}~\cite{DRACO}) or place a heavy computation overhead on the PS (such as
\bulyan{}~\cite{guerraoui2018hidden}). Furthermore, they introduce a heavy communication overhead. \cite{detox2019} interpolates between \draco{} and robust aggregation methods for faster computation on both compute nodes and the PS. However, it does not mitigate the communication bottleneck, whereas \solon{} introduces both black-box Byzantine-resilience guarantee and communication-efficiency. 

Communication-efficient distributed machine learning has gained a lot of attention. Various methods propose to use gradient compression, \eg via quantization~\cite{seide20141,alistarh2016qsgd,wen2017terngrad,suresh2017distributed} or sparsification~\cite{stich2018sparsified,Wang18Atomo,lin2017deep,vogels2019powersgd,agarwal2020accordion} to enhance the communication efficiency. These methods massively compress the gradients, however, their Byzantine-resilience is not clear.

The methods that are the most similar to \solon{} are \signum{}~\cite{bernstein2018signsgd} and the one proposed in~\cite{ghosh2020communication}. These methods introduce both communication-efficiency and Byzantine-resilience, however their Byzantine-resilience guarantees are not as strong as for \solon{} in theory, i.e. they typically use lossy compression for coding and decoding schemes, which only achieve approximated recovery under certain attacks.  

==> Solon_Arxiv (5)/Figure/Theory.tex <==

\section{\solon{}}
\label{sec:solon}
	\vspace{-0.1in}

In this section we give an overview of the \solon{} framework, discuss constraints on the encoding and decoding functions, and define optimal coding schemes.

The proofs are left to the appendix.

\subsection{Preliminaries}	\vspace{-0.1in}

\paragraph{Basic notations.}
For a matrix $\mathbf{A}$, let $\mathbf{A}_{i,j}$, $\mathbf{A}_{i,\cdot}$, and $\mathbf{A}_{\cdot, j}$ denote entries, rows, and columns, respectively. More generally, $\mathbf{A}_{S,T}$ is the submatrix of $\mathbf{A}$ with rows indexed by  $S$ and columns indexed by $T$. The Hadamard, or elementwise, product $\mathbf{A} \odot \mathbf{B}$ of two matrices of the same size has entries $(\mathbf{A}\odot \mathbf{B})_{i,j} = \mathbf{A}_{i,j}\mathbf{B}_{i,j}$. Let $m$ be the dimension of the data, $n$ be the size of the training set, and $\mathbf{x}_i\in\mathbb{R}^m$, $i=1,\ldots,m$ be the data points. Let $\ell(\cdot;\cdot)$ be the loss function, $d$ be the model dimension, and ${\bf w}\in\mathbb{R}^d$ be the model parameters.  Let $\mathbf{1}_m$ and $\mathbf{1}_{n\times m}$ be the $m\times 1$ vector, and $n\times m$ matrix, of all ones, respectively. Similarly, let $\mathbf{0}_{m}, \mathbf{0}_{n\times m}$ contain zeros.  The empirical risk minimization (ERM) \cite{NIPS1991ERM,vapnik2013nature} objective is: 
$\min_{{\bf w}} {n}^{-1}\sum_{i=1}^n \ell({\bf w};\mathbf{x}_i).$
The most common current approach is to use first-order stochastic optimization to solve this, in particular mini-batch stochastic gradient descent (SGD). Starting at an initial point ${\bf w}_0$, we iterate 
${\bf w}_k = {\bf w}_{k-1} - \gamma/|S_k| \sum_{i \in S_k}\nabla\ell_{\bf w}({\bf w}_{k-1}; \mathbf{x}_{i}),$
where $S_k \subseteq \{1,\ldots, n\}$ is a random subset of size $B$ and $\gamma>0$ is the learning rate.

We relabel $S_k$ to $\{1,\ldots, B\}$ and denote $\nabla \ell({\bf w}_{k-1};\mathbf{x}_i)$ by $\mathbf{g}_i$. 

\paragraph{Distributed learning.}
We aim to compute $\mathbf{g}=\sum_{i = 1}^B \mathbf{g}_i$ in a distributed, {\it adversary-resistant}, and {\it communication efficient} manner. We consider a distributed training model where gradient computations are partitioned across $P$ compute nodes at each iteration. These operate on a potentially reduced dimension $d_c$ for communication efficiency, and we let the gradient \emph{compression ratio} be $\smash{r_c \triangleq d/d_c}$. After computing and summing up their assigned gradients, each node sends their answer back to the parameter server (PS). This sums them and updates the model. By applying \solon{}, we reduce the communication complexity for sending gradients to server from $\mathcal{O}(Pd)$ to $\mathcal{O}(Pd_c)$. The broadcast phase of sending aggregated gradients from server to compute nodes takes $\mathcal{O}(\log{(P)}d)$, which is not the major overhead. 

\eat{
\vspace{0.1in}
\begin{remark}
	Compared to previous works, our analysis and framework are applicable to any distributed algorithm which requires the sum of multiple functions. Notably, 
the framework can be applied to any first-order methods, including gradient descent, SVRG \cite{johnson2013accelerating}, coordinate descent, and projected or accelerated versions of these algorithms. 
	For the sake of simplicity, our discussion in the rest of the paper will focus on mini-batch SGD.
\end{remark}
}
We assume that at most $s$ compute nodes are unreliable, Byzantine, or adversarial, and can send to the PS an arbitrary update. 

We consider the strongest possible adversaries: with infinite computational power, knowing the entire data set, the training algorithm, any defenses present in the system, and able to collaborate.

\subsection{Framework}	\vspace{-0.1in}
\solon{} is defined by the tuple, or \emph{mechanism}, $(\mathbf{A}, E, D)$, where $\mathbf{A}$ is an allocation matrix specifying how to assign gradients to nodes, $E$ are encoding functions determining how each compute node should locally encode its gradients, and $D$ is a decoding function determining how the PS should decode the output of the nodes. As an example, in Figure \ref{fig:RunningExample}(a), $A$ corresponds to the gradient computation assignment of the compute nodes, $E$ corresponds to the summation of the gradients by each node, and $D$ refers to the decoding phase at the PS. 
We generalize the scheme in Figure \ref{fig:RunningExample} to $P$ compute nodes and $B$ gradients. % \scream {should not say data samples, but gradients?}.

{\bf Allocation matrix, $\mathbf{A}$.} 
At each iteration of the training process, we assign the $B$ gradients to the $P$ compute nodes using a $P\times B$ {\it allocation matrix} $\mathbf{A}$, where $\mathbf{A}_{j,k}$ is equal to unity ("1") if node $j$ is assigned to the $k$th gradient ${\bf g}_k$, and zero ("0") otherwise. The support of $\mathbf{A}_{j,\cdot}$, denoted $\supp\left(\mathbf{A}_{j,\cdot}\right)$, is the set of indices of gradients evaluated by the $j$th node. For simplicity, we will assume $B=P$. % throughout the following.
Let $\|\mathbf{A}\|_0$ be to the $L_0$ norm of a matrix, i.e., the number of nonzero entries.
Following \cite{DRACO}, we define the \emph{redundancy ratio} of an allocation as the average number of gradients assigned to each compute node, or equivalently $r\triangleq  \|\mathbf{A}\|_0/P$.

We define the $d \times P$ matrix $\mathbf{G}$ with gradients as its columns: $\mathbf{G} \triangleq [\mathbf{g}_1,\mathbf{g}_2,\cdots, \mathbf{g}_P]$. The $j$th node first picks out its assigned gradients using the allocation matrix $\mathbf{A}$, computing a $d\times P$ gradient matrix $\smash{\mathbf{Y}_j \triangleq \left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}}$. 
The columns of this matrix are $\mathbf{g}_k$ if the $k$th gradient $\mathbf{g}_k$ is allocated to the $j$th compute node, \ie $\mathbf{A}_{j,k} \not = 0$, and zero otherwise.

{\bf Encoding Functions, $E$.} The $j$th compute node is equipped with an encoding function $E_j$ that maps the $d\times P$ matrix $\mathbf{Y}_j$ of its assigned gradients to a $d_c$-dimensional vector.
The $j$th compute node computes and sends $\smash{\mathbf{z}_j \triangleq E_j(\mathbf{Y}_j)}$ to the PS.
If the $j$th node is adversarial, then it instead sends $\smash{\mathbf{z}_j+\mathbf n_{j}}$ to the PS, where $\mathbf n_{j}$ is an arbitrary $d_c$-dimensional \emph{Byzantine} vector.
We let  $E = \{ E_1, E_2, \cdots, E_P\}$ be the set of local encoding functions.

{\bf Decoding Function, $D$}. The $d_c \times P$ matrix $\smash{\mathbf{Z}=\mathbf{Z}^{\mathbf{A},E,\mathbf{G}} \triangleq [\mathbf{z}_1, \mathbf{z}_2,\cdots, \mathbf{z}_P]}$ contains all outputs of the nodes. The $d_c \times P$ matrix $\smash{\mathbf{N} \triangleq [\mathbf{n}_1, \mathbf{n}_2,\cdots, \mathbf{n}_P]}$ contains all Byzantine vectors, with at most $s$ non-zero columns.
Then, the PS receives a $d_c\times P$ matrix $\smash{\mathbf{R} \triangleq \mathbf{Z} +\mathbf{N}}$, and computes a $d$-dimensional vector $\smash{\mathbf{u} \triangleq D(\mathbf{R})}$ using a decoding function $D$.


We require that the algorithm at the PS recovers the $d$-dimensional sum of gradients, $\mathbf{G} \mathbf{1}_P$:

\begin{definition}
	\solon{} with $(\mathbf{A}, E, D)$ can tolerate $s$ adversarial nodes, if for any $\mathbf{N} = [\mathbf{n}_1,\mathbf{n}_2,\cdots, \mathbf{n}_P]$ such that $ \left\vert{ \{j:\mathbf{n}_{j}\not=0\} }\right\vert \leq s$, we have $D(\mathbf{Z}+\mathbf{N}) = \mathbf{G}\mathbf{1}_P$.
\end{definition}

If we defend against the Byzantine attack, then the model update at each iteration is identical to the adversary-free setting. 
This implies that  convergence guarantees for the adversary-free case transfer to the adversarial case.

\subsection{Encoding and decoding functions}	\vspace{-0.1in}
What are the fundamental limits of the above allocation, encoding, and decoding schemes, in particular of the redundancy ratio used in allocation and the compression ratio used in encoding?  Perhaps surprisingly, \emph{the redundancy ratio does not depend on the compression ratio}.
The encoded gradients at each compute node can be arbitrarily compressed without affecting the our ability to tolerate Byzantine attacks.
The reason is that any $d$-dimensional real vector can be mapped one-to-one to a real number. This is stated in the following theorem.

\begin{theorem}\label{Thm:GenericBound}
	If there is a mechanism $(\mathbf{A}, E, D)$ of gradient allocation, encoding, and decoding with redundancy ratio $r$ tolerating $s$ adversarial nodes with a compression ratio $r_c$ of unity, then there is a mechanism $(\mathbf{A}', E', D')$ with redundancy ratio $r$ tolerating $s$ adversarial nodes for any compression ratio $r_c>0$.
\end{theorem}


However $(\mathbf{A}', E', D')$ is in a sense pathological and it is unclear if it can reduce the the number of bits communicated.
Therefore, we seek classes of \textit{regular} encoder and decoder functions $E,D$, to reduce communication cost.

\begin{definition}
	 A set of encoding functions $E$ is called {\em regular} if each output element of each function $E_j$ is a function of linear combinations of columns of the input. Formally, if $E_{j,v}$ is the $v$th element of $E_j$, then
	 $(\mathbf{A}, E, D)$ is regular if there exists a $d\times P$ matrix $\mathbf{U}_{j,v}$ and functions $\smash{\hat{E}_{j,v}}$, such that $\smash{E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}\left(\mathbf{1}_d^T\left(\mathbf{U}_{j,v} \odot \mathbf{Y}_{j}\right)\right)}$.
\end{definition}

%To better understand the \textit{regular} condition, 
When $d=1$, $\mathbf{Y}_j$ has only one row and $\mathbf{1}_{d}=1$ is a scalar.
Thus, $E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}(\mathbf{U}_{j,v} \odot \mathbf{Y}_j)$ implies that $E$ is an arbitrary function of $\mathbf{Y}_j$.
When $d>1$, each output coordinate only depends on linear combinations of input columns.
Since linear combinations do not introduce extra bits, this allows practical communication compression. We will study regular encoders $E$.

\paragraph{Redundancy Bound.}
We first study redundancy requirements for exact recovery of the sum of gradients with $s$ adversaries and compression ratio $r_c$. 
\begin{theorem}\label{Thm:RedundancyRatioBound}
A mechanism $(\mathbf{A}, E, D)$ of gradient allocation, regular encoding, and decoding with compression ratio $r_c$ tolerating $s$ adversarial nodes must have a redundancy ratio $r \geq 2s+r_c$.
\end{theorem}

Thus, for any regular encoder, each gradient has to be replicated on average at least $2s+r_c$ times to defend against $s$ adversarial nodes with a communication compression ratio of $r_c$. If a mechanism tolerates $s$ adversarial nodes with a communication compression ratio of $r_c$, by Theorem \ref{Thm:RedundancyRatioBound}, each compute node encodes at least $(2s+r_c)$ $d$-dimensional vectors on average. If the encoding has linear time complexity, then each encoder requires $O((2s+r_c)d)$ operations in the worst case. If the decoder $D$ has linear time complexity, then it requires at most $O(Pd_c)$ operations in the worst case, as it needs to use the $d$-dimensional input from all $P$ compute nodes. This gives a computational cost of $O(Pd_c)$, which is less than the bound $\mathcal{O}(Pd)$  for the repetition code in \cite{DRACO}.

To better understand the lower bound, we give an equivalent formulation it in the language of linear algebra. Let $g$ be one of the $d\times 1$ dimensional gradients. Suppose it gets sent to $r$ nodes. Then the potentially  corrupted output of the linear encoder at each node $j$  can be represented by $R_j = Z_j g + n_j$, and $n_j$ is the noise here for $j=1,\ldots, r$, where each $Z_j$ is a $d_c \times d$ dimensional matrix. If the number of adversaries is at most $s$, then at most $s$ vectors $n_j$ are nonzero. We call this set of perturbation $B_{s,r}$. Thus, the goal is to design the $r$ matrices $Z_j$, such that for any collection of vectors $n_j$ at most $s$ of which are nonzero, it is possible to recover $g$ from the observations $(Z_j,r_j)$, $j=1,\ldots, r$.
Let $R:=(R_1,\ldots, R_r)$ and $n:=(n_1,\ldots,n_r)$, which we view as a concatenation of vectors belonging to the allowed set $B_{s,r}$. For the recovery of $g$ to be possible, we need that if $R(g,n) = R(g',n')$ for $g,g'\in \R^d$ and $n,n'\in B_{s,r}$, then $g=g'$. 

We can write $R$ as a linear function $R = Zg+n$, where $Z$ is an $rd_c\times d$ concatenation of the matrices $Z_i$. Thus, we can write $R(g,n) = R(g',n')$ as
$Zg+n=Zg'+n' \iff Z(g-g')=n-n'.$
Moreover, we have $n''  = n-n' \in B_{2s,r}$, because at  most $2s$ of its $P$ sub-vectors of size $d_c$ are nonzero. Clearly, all vectors in $B_{2s,r}$ can be written in this form.  Denoting $x = g-g'$, the problem is to understand when there exists a matrix $Z$ such that for all $x \in \R^d$, we have $Zx \notin B_{2s,r}$. Now, $B_{2s,r}$ is a union of several $2sd_c$-dimensional linear subspaces in $rd_c$ dimensions. Moreover, $Zx$ belongs to $span(Z)$, which is an at most $d$-dimensional subspace in $rd_c$ dimensions. Thus, for this to be possible, by counting dimensions we obtain that we need $rd_c\ge 2sd_c +d$. Since $r_c=d/d_c$, this is equivalent to $r\ge 2s +r_c$. This finishes the proof of the fundamental lower bound on the redundancy.



\subsection{Optimal Coding Schemes}
\label{ocs}
%\paragraph{Optimal Coding Schemes}
	\vspace{-0.1in}
Can we achieve the optimal redundancy bound with linear-time encoding and decoding? 
More formally, can we design a tuple $(\mathbf{A},E,D)$ with redundancy ratio $r=2s+r_c$ and computation complexity $\mathcal{O}((2s+r_c)d)$ at the compute nodes and $\mathcal{O}(Pd_c)$ at the PS?
We give a positive answer by designing certain {\em linear block codes} that match the above bounds. 


This is a challenging problem. In fact, we can show (see Appendix \ref{sp}) that this question is \emph{exactly equivalent to a sparse recovery problem}, where we wish to recover an unknown sparse vector from linear combinations of a fixed set of vectors \cite{chen1994basis,chen2001atomic,elad2010sparse}. 
With this lens, our algorithms are related to the classical Prony's method in signal processing \cite{hurst1987scattering,Prony}. However, a key difference is that in our case, we have a \emph{structured set of perturbations}, where entire sub-vectors corresponding to gradients are perturbed at the same time. We leverage this to develop algorithms faster than Prony's method.
\vspace{-0.1in}
\paragraph{Linear Block Code.} 

We focus on the case when $2s+r_c$ divides $P$; otherwise we can change $P$ or $r_c$ until $2s+r_c$ divides $P$. 
Divide the compute nodes into $q:=P/(2s+r_c) = P/r$ ``blocks'' or groups.
We assign each node in the same block to compute the same gradients. 
Each node sends some linear combination of coordinates of the assigned gradients to the PS (``linear'').
The PS solves systems of linear equations to get the desired gradient sum.  
Following the convention of coding theory \cite{abclbc}, we call our approach \textit{linear block codes}.

The linear block code $(\mathbf{A}, E, D)=(\mathbf{A}^{LBC}, E^{LBC}, D^{LBC})$ is defined as follows. 
The assignment matrix is $\mathbf{A} = \mathbf{I}_q \otimes \mathbf{1}_{r \times r}$.

The $j$th compute node first selects its allocated gradients $\mathbf{Y}_j=\left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}$.
Its encoder function sums up the allocated gradients into $\mathbf{Y}_j \mathbf{1}_P$, then computes and sends $\mathbf{z}_j = E_j(\mathbf{Y}_j) = \mathbf{W}_j \mathbf{Y}_j\mathbf{1}_P$  to the PS, where $\mathbf{W}_j$ is a $d_c \times d$ matrix. 
%That is, It then sends $\mathbf{z}_j = E_j^{\mathit{Rep}}(\mathbf{Y}^{Rep}_j)$.

The decoder function, summarized in Algorithm \ref{Alg:DecoderFunction_LinearBlock}, partitions the received updates into the $q$ blocks computing identical gradients.
For each, a block decoder $\psi(\cdot,\cdot)$ is called to recover the sum of all gradients in this group.
\vspace{-0.1in}
\begin{algorithm}[htbp]
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{Received $d_c \times P$ matrix $\mathbf{R}$}
	\Output{Desired gradient summation $\mathbf{u}$}
	Let $\mathbf{R} = \left[\mathbf{R}_1, \mathbf{R}_2, \cdots, \mathbf{R}_{q}\right]$, where each $\mathbf{R}_j$ is a $d_c\times r $ matrix
	
    \For{$j=1$ \KwTo $q$ }
    {
         \textrm{ } $ V = \phi(\mathbf{R}_j,j)$ // Locate the adversarial nodes\\
		$U = \{1,2,\cdots,r\} \setminus V$ // Non-adversarial nodes\\
    $\mathbf{u}_j = \psi(\mathbf{R}_j,j, U)$ // Decode each block using the non-adversarial nodes
    }
	%into $d_c\times r$ matrices
	Compute and return $\mathbf{u} = \sum_{i=1}^{q}\mathbf{u}_i$
	\caption{Decoder Function $D$.}
	\label{Alg:DecoderFunction_LinearBlock}
\end{algorithm}
% \vspace{-0.1in}

There are three questions left: (i) how $\mathbf{W}_j$ is constructed, (ii) how the adversarial node index location function $\phi(\cdot)$ works, and (iii) how the block decoder function $\psi(\cdot,\cdot)$ works.


Given any distinct nonzero scalars $w_1, w_2, \cdots, w_P$, we propose to construct $\mathbf{W}_j$ as $\mathbf{W}_j \triangleq \mathbf{I}_{d_c}\allowbreak$ $\otimes [\allowbreak1,\allowbreak w_j,\allowbreak w_j^2,\allowbreak \cdots,\allowbreak w_j^{r_c-1}]$. The adversarial node index locating function $\phi(\cdot)$ works as follows.
Given the $d_c \times r$ matrix $\mathbf{R}_j$ received from the compute nodes, we first generate a $1\times d_c$ random vector $ \mathbf{f} \sim \mathcal{N}(\mathbf{1}_{1\times d_c},\,\mathbf{I}_{d})$,
and then compute $\smash{\mathbf{r}_{j,c} \triangleq \mathbf{f} \mathbf{R}_j}$.
Next, we obtain an $r$-dimensional vector $\mathbf{a} = [a_1, a_2,\cdots, a_{r}]$ by  solving the linear system
$\begin{bmatrix}
     \hat{\mathbf{W}}_{j,r_c+s-1},\allowbreak  & -\hat{\mathbf{W}}_{j,s-1} \odot\allowbreak \left( \mathbf{r}_{j,c}^T \mathbf{1}_{s}^T\right)
\end{bmatrix}
    \mathbf{a}= \mathbf{r}_{j,c} \odot \left[\hat{\mathbf{W}}_{j,s}\right]_{\cdot,s}$,
 where 
	\[
\hat{\mathbf{W}}_{\mathit{j},v} \triangleq
\begin{bmatrix}
1 & w_{(j-1)r+1} &  w_{(j-1)r+1}^2 &\cdots &  w_{(j-1)r+1}^{v} \\
1 & w_{(j-1)r+2} &  w_{(j-1)r+2}^2 &\cdots &  w_{(j-1)r+2}^{v} \\
\vdots & \vdots & \vdots & \vdots & \vdots\\
1 & w_{jr} &  w_{jr}^2 &\cdots &  w_{jr}^{v}
 \\
\end{bmatrix}.
\\
\]
Finally compute $P_j(w) \triangleq (\sum_{i=0}^{r_c+s-1} a_{i+1} w^i)/(w^s+\sum_{i=0}^{s-1} a_{i+r_c+s+1} w^i) $,
and return $V=\{i|P_j(w_{(r-1)j+i}) \not =\left[ \mathbf{r}_{j,c}\right]_i\}$.
The decoding function $\psi(\cdot, \cdot)$ computes and returns $\textit{vec}\left(\left[\mathbf{R}_{j}\right]_{\cdot, U} \left[\hat{W}_{j,r_c-1}\right]_{U,\cdot}^{-1,T}\right)$ given the non-adversarial node indices $U$.

The following lemma ensures that the Byzantine nodes are correctly found.
\begin{lemma}\label{Thm:LBCDetection}
	Suppose $\left\vert{\{j:\|\mathbf{n}_{j}\|_0 \not=0\}}\right\vert$ $\leq s$ and $r\geq r_c+2s$. 
	Then $\phi(\mathbf{R}_j,j) =  \{i:\|\mathbf{n}_{j(r-1)+i}\|_0 \not=0\}$ with probability equal to unity. 
\end{lemma}
The next lemma demonstrates that within each group the gradient is correctly recovered.
\begin{lemma}\label{thm:LBClocalcorrect}
	If $U$ consists solely of at least $r-s$ non-adversarial nodes, then  with probability equal to unity, $\mathbf{u}_j = \sum_{k=(j-1)r+1}^{jr}\mathbf{y}_{k}$.
\end{lemma}

Combing the above two results,  we show that the linear block code tolerates any $s$ adversaries, achieving the optimal redundancy and compression ratio with linear-time encoding and decoding.

\begin{theorem}\label{Thm:LinearBlockCodeOptimality}
	The linear block code  $(\mathbf{A}, E, D)$ tolerates any $s$ adversaries with probability equal to unity, and achieves the redundancy ratio  bound. For $d\gg P$, its encoding and decoding achieve linear-time computational complexity. 
% \ed{clarify}
\end{theorem} 

Theorem \ref{Thm:LinearBlockCodeOptimality} shows that the linear block code is information theoretically tight and enjoys a small computational overhead even for large ML models. 
 


==> Solon_Arxiv (5)/Figure/macros.tex <==
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{amsthm,amsmath,amssymb}
%\usepackage{graphicx,xspace,verbatim,comment}
%\usepackage{array,color,multirow}
%\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{float,url,amsfonts,alltt}
\usepackage{mathtools,rotating}
\usepackage{ifpdf,fancyvrb}
\usepackage{enumitem}
%\usepackage{algorithm,algpseudocode}
%\usepackage{etoolbox,listings,subcaption}
%\usepackage{bigstrut,morefloats}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
%\usepackage{thm-restate}
%\usepackage{todonotes}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
\usepackage{subfigure}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}

\usepackage{graphicx,xspace,verbatim,comment}
\usepackage{hyperref,array,color,balance,multirow}
\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{mathtools,rotating,amsmath,amssymb}
\usepackage{color,ifpdf,fancyvrb,array}
% \usepackage{algorithm,algpseudocode}
\usepackage{etoolbox,listings}
%\usepackage{subcaption}
\usepackage{bigstrut,morefloats}
\usepackage{makecell}
%\usepackage[boxruled]{algorithm2e}
\usepackage{pbox}
\usepackage[numbers]{natbib}
\usepackage{algorithm, algorithmic}
\usepackage[boxruled,algo2e,linesnumbered]{algorithm2e}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newcommand{\eat}[1]{}

\newcommand{\gaussian}[2]{\mathcal{N}(#1,#2)}


% User Defined Commands
\newcommand{\systemnameSolon}{\textsc{Solon}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\cmp}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\detox}{\textsc{Detox}}
\newcommand{\draco}{\textsc{Draco}}
\newcommand{\solon}{\textsc{Solon}}
\newcommand{\bulyan}{\textsc{Bulyan}}
\newcommand{\multikrum}{\textsc{Multi-Krum}}
\newcommand{\signum}{\textsc{Signum}}
% \newcommand{\eg}{\textit{e.g., }}
% \newcommand{\ie}{\textit{i.e., }}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\hier}{\textsc{Hier-Aggr}}
%
\newcommand{\lingjiao}[1]{{\color{blue} {\bf Lingjiao:} #1}}
\newcommand{\leshang}[1]{{\color{red} {\bf Note:} #1}}

\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\indi}{\mathds{1}}
\newcommand{\ie}{{\emph i.e.,} }
\newcommand{\eg}{{\it e.g.}, }
\newcommand{\tr}{\operatorname{tr}}
% \newcommand{\R}{\mathbb{R}}
%\newcommand{\C}{\mathbb{C}}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\cov}{\operatorname{Cov}}
% \newcommand{\PP}{\mathbb{P}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecwb}{\mathbf{w}}
\newcommand{\tvecw}{\widetilde{\mathbf{w}}}
\newcommand{\tvecwb}{\widetilde{\mathbf{w}}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\ovecv}{\overline{\mathbf{v}}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\tvecz}{\widetilde{\mathbf{z}}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\gradf}{\nabla f}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\gradtf}{\nabla \widetilde{f}}
\newcommand{\gradF}{\nabla F}
\newcommand{\HW}{\textsc{Hogwild!}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\const}{\mathcal{O}(1)}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\CM}{\textsc{KroMagnon}}
\newcommand{\cdeg}{\overline{\Delta}}
\newcommand{\ct}{\mathcal{O}(1)}
\newcommand{\W}{\mathcal{W}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norms}[1]{\|#1\|}
\newcommand{\twonm}[1]{\left\|#1\right\|_2}
\newcommand{\twonms}[1]{\|#1\|_2}
\newcommand{\onenm}[1]{\left\|#1\right\|_1}
\newcommand{\onenms}[1]{\|#1\|_1}
\newcommand{\fbnorm}[1]{\left\|#1\right\|_F}
\newcommand{\fbnorms}[1]{\|#1\|_F}
\newcommand{\prob}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\probs}[1]{\mathbb{P}\{#1\}}
\newcommand{\EXP}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\EXPS}[1]{\mathbb{E}[#1]}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\innerp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\innerps}[2]{\langle#1,#2\rangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\abss}[1]{|#1|}
\newcommand{\tsp}{^{\rm T}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\mt}{B\floor{t/B}}
%\newcommand{\G}{\overline{G}}
%\newcommand{\B}{\overline{B}}
\numberwithin{equation}{section}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\red}[1]{{\color{red}{#1}}}

\newcommand{\paris}[1]{{\color{red} #1}}


\newcommand\overmat[2]{%
	\makebox[0pt][l]{$\smash{\color{white}\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{\color{black}#1}}}$}#2}
\newcommand\bovermat[2]{%
	\makebox[0pt][l]{$\smash{\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{#1}}}$}#2}
					
\newcommand\bundermat[2]{%
	\makebox[0pt][l]{$\smash{\underbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}_{\text{#1}}}$}#2}
					
					
\newcommand\partialphantom{\vphantom{\frac{\partial e_{P,M}}{\partial w_{1,1}}}}

\newcommand{\scream}[1]{{\bf * #1 *}{\typeout{#1}}}

\usepackage{amsmath}
\usepackage{accents}
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
    
%\usepackage{algorithm,algpseudocode}


\newtheorem{theo}{Theorem}
\newtheorem{introtheo}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{rem}{Remark}
\newtheorem{asm}{Assumption}
\newtheorem{example}{Example}
\newtheorem{property}{Property}

\newcommand{\blkdiag}{\text{blkdiag}}
\newcommand{\GGG}{{\color{red}{\bf [GGG CHECK]}}}
\newcommand{\sort}{\text{sort}}
\newcommand{\Span}{\text{span}}
\newcommand{\supp}{\text{supp}}
\newcommand{\bsp}{\hspace{-0.14cm}}
\newcommand{\T}{\intercal}
\newcommand{\eqdef}{\stackrel{\triangle}{=}}
\newcommand{\G}{ \mathcal{G} } 
\newcommand{\Gnp}{ \mathcal{G}\left(n,\frac{1}{2}\right) } 
\newcommand{\Gnpk}{ {G}\left(n,\frac{1}{2}, k\right) }
\newcommand{\opt}{\textsf{opt}}
\newcommand{\A}{{\bf A}}
\newcommand{\den}{\textsf{den}}
\usepackage[T1]{fontenc}
\usepackage{upgreek}

\newcommand{\Exp}{\mathbb{E}}
\usepackage[greek,english]{babel}
% \usepackage[utf8x]{inputenc}
\usepackage{pifont}
\usepackage{float}
\usepackage{autobreak}


==> Solon_Arxiv (5)/Introduction.tex <==
\section{Introduction}\label{Sec:SOLON:Intro}
The growing size of datasets and machine learning models has led to many developments in distributed training using stochastic optimization~\cite{devlin2018bert,deng2009imagenet,sergeev2018horovod,dean2012large,dobriban2020wonder}.
One of the most widely used %distributed training
settings is the {\em parameter server (PS) model}~\cite{li2013parameter,li2014scaling,jiang2020unified}, 
where the gradient computation is partitioned among all compute nodes, typically using stochastic gradient descent (SGD) or its variants. A central parameter server then aggregates the calculated gradients from all compute nodes to update the global model. 



However, scaling PS models to large clusters introduces two challenges: guarding against \textit{Byzantine attacks} and managing  \textit{communication overhead}.
Byzantine attacks include erroneous gradients sent from unreliable compute nodes due to power outages, hardware or software errors, as well as malicious attacks. 
The communication overhead of sending gradients to the PS in large clusters can also be extremely high, potentially dominating the training time, ~\cite{dean2012large,alistarh2017qsgd,wen2017terngrad,Wang18Atomo, DRACO}, since the number of gradients sent is linear in the number of compute nodes. 

Although recent work has studied the problem of
Byzantine attacks under the PS model~\cite{ALIE2019,guerraoui2018hidden,xie2020fall}, the communication overhead remains prohibitive. For example, ~\cite{blanchard2017machine,chen2017distributed,yin2018byzantine,AggregathorDamaskinosEGGR19} use {\em robust aggregators} at the PS to mitigate  unreliable gradients, 
while ~\cite{DRACO} introduces {\em algorithmic redundancy} to detect and remove Byzantine nodes. 
Robust aggregators are computationally
expensive due to their super-linear  (often quadratic) dependence on the number
of nodes. They also often have limited convergence guarantees under
Byzantine attacks, e.g., only establishing convergence in the limit, or only guaranteeing that the output of the aggregator has a positive inner product with the true gradient. 
They often require strong bounds on the dimension of the model.
Although algorithmic redundancy or coding-theoretic~\cite{Gradient_Coding, DRACO}
approaches offer strong convergence guarantees, these approaches have high communication overhead.

Thus, it remains an open question to simultaneously provide \textbf{\emph{Byzantine-resilience with strong guarantees and communication efficiency}} for distributed learning.


\begin{figure*}[t] 
\centering
\subfigure[Example of a \solon{} instance]{\includegraphics[width=0.6\textwidth]{Figure/intro_fig_2.pdf}}
% \hfill
\hskip 5pt
\subfigure[Performance of \solon{}]{\includegraphics[width=0.37\textwidth]{Figure/accu_hour_3000_revgrad_node50_ResNet_w_errorbar.pdf}}
\vspace{-2mm}
\caption{\footnotesize{Demonstration of \solon{}. (a) gives an example of \solon{}, where the cluster consists of  four compute nodes.  (b) shows the runtime performance of \solon{} $r_c=10$ when training ResNet-18 on CIFAR-10 under rev-grad attack. Compared to various baselines, \solon{} converges faster and provides higher final accuracy.}}
\label{fig:RunningExample}
% \vspace{-2mm}
\end{figure*}

To address this problem, we propose \solon{}, a distributed training framework leveraging algorithmic redundancy to protect against Byzantine attacks, and ideas from sparse recovery~\cite{Prony} and coding theory~\cite{Gradient_Coding} to reduce communication overhead. 
The approach is as follows: 
In a Byzantine-free PS model with $P$ compute nodes and $B$ gradients to be computed, at each iteration
each of the $P$ nodes computes $B/P$ gradients, and sends them to the PS.  In \solon{}, gradients are computed redundantly to tolerate Byzantine failures; each node computes $rB/P$ gradients, incurring a {\em computational redundancy ratio} of $r$.  To reduce communication overhead, compressed gradients are sent to the PS.  For $d$-dimensional gradients, each node only sends a $d/r_c$-dimensional vector to the PS, where  $r_c$ is the {\em compression ratio}. 

We show that under worst-case adversarial conditions where the adversarial nodes have access to the complete data and gradients, and can send arbitrary results to the PS, there is a fundamental trade-off among Byzantine-resilience, communication overhead and computation cost. To tolerate $s$ Byzantine nodes, the redundancy ratio must satisfy $r\geq 2s+r_c$.
We provide a concrete encoding and decoding technique for \solon{} based on Vandermonde matrices and building on Prony's method from signal processing ~\cite{Prony,communciation_gradcoding_min_ye} that matches the optimal condition  $r= 2s+r_c$. 


\paragraph{Example.}
Figure \ref{fig:RunningExample}(a) shows
four two-dimensional gradient vectors, $g_1, g_2,g_3, g_4$, where gradients $g_i=(g_{i1},g_{i2})$ are in different colors.
To tolerate Byzantine workers, 
each node computes four gradients. 
However, instead of sending a two-dimensional vector to the PS, each node only sends a one-dimensional linear combination of the elements in the local gradients. For instance, worker 1 computes and sends the scalar $g_{11}+g_{12}+g_{21}+g_{32}+g_{41}+g_{42}$. Here, the redundancy ratio $r=4$ and the compression ratio $r_c=2$. The PS uses a decoding scheme presented in Section \ref{sec:solon}. Therefore \solon{} can recover the correct gradient with one Byzantine worker ($4 \geq 2\times 1 + 2$). 
\qed


We implemented \solon{} in Pytorch and conducted extensive experiments on a large cluster.  Our results show that
\solon{} can provide significant speedups across various ML models and datasets over existing methods, such as \bulyan{} \cite{guerraoui2018hidden} and \draco{}~\cite{DRACO}, shown in Figure \ref{fig:RunningExample}(b) using ResNet-18~\cite{ResNet} on CIFAR-10~\cite{Cifar10} under a reverse gradient attack. 
In addition, 
\solon{} successfully defends against strong Byzantine attacks such as ``A little is enough'' (ALIE)~\cite{ALIE2019}, on which some methods such as \bulyan{} and \signum{} \cite{bernstein2018signsgd} fail to converge or result in significant accuracy loss, see Section \ref{Sec:SOLON:Experiment}. 

\vspace{-0.1in}
\paragraph{Contributions.}   Our contributions include:
\vspace{-0.1in}
\begin{enumerate}
    \item \solon{}, a distributed training framework that exploits algorithmic redundancy to simultaneously provide Byzantine-resilience and communication efficiency. 
    \vspace{-0.07in}
    \item A concrete encoding and decoding mechanism, which is provably efficient and  achieves the optimal trade-off between Byzantine resilience, communication overhead, and computational cost.  
    % \vspace{-0.07in}
    \item Extensive experiments which show that \solon{} exhibits significant speedups as well as strong Byzantine-resilience over previous approaches.   
\end{enumerate}

The \solon{} framework can be used for any distributed algorithm which requires the sum of multiple functions, including gradient descent, SVRG \cite{johnson2013accelerating}, coordinate descent, and projected or accelerated versions of these algorithms. However, in this paper, we focus on mini-batch SGD.
The rest of the paper is organized as follows: Section \ref{Sec:SOLON:relatedwork} discusses related work. 
Section \ref{sec:solon} presents the \solon{} framework and theoretical guarantees. Experimental results are given in Section \ref{Sec:SOLON:Experiment}. 

\section{Related work}
\label{Sec:SOLON:relatedwork}
Byzantine fault tolerance against worst-case and/or adversarial failures such as system crashes, power outages, software bugs, and adversarial agents that exploit security flaws has been extensively studied since the 1980s~\cite{lamport2019byzantine}. In distributed machine learning, these failures may appear when a subset of compute nodes returns to the PS erroneous updates. It is well understood that first-order methods, such
as gradient descent or mini-batch SGD, are not robust to Byzantine errors; even a single erroneous update can introduce arbitrary errors to the optimization variables~\cite{blanchard2017machine,chen2017distributed}. At the same time, distributed model training suffers from communication overhead due to frequent gradient updates transmitted between compute nodes~\cite{LargeScaleDeepNet_Dean12,mcmahan2017communication,li2014communication,konevcny2016federated,dobriban2020wonder,dobriban2021distributed}. \solon{} aims at improving both Byzantine-resilience and communication-efficiency in distributed model training.

More recently, attention has turned to Byzantine-resilient distributed machine learning techniques.  Results show that while average-based gradient methods are susceptible to adversarial nodes, robust gradient aggregation methods can, in some cases, achieve better convergence while being robust to some attacks~\cite{chen2017distributed,el2019sgd,blanchard2017machine,xie2018zeno,xie2020fall,blanchard2017machine,yin2018byzantine,guerraoui2018hidden,jaggilearningfromhistory}. Despite
theoretical guarantees, the proposed algorithms often only ensure
a weak form of resilience against Byzantine failures, and can fail against strong Byzantine attacks~\cite{guerraoui2018hidden,xie2020fall,ALIE2019}. Another line of work proposes to use algorithmic redundancy to attain black-box Byzantine-resilience guarantees. However, many of these techniques require redundant computation from compute nodes (such as \draco{}~\cite{DRACO}) or place a heavy computation overhead on the PS (such as
\bulyan{}~\cite{guerraoui2018hidden}). Furthermore, they introduce a heavy communication overhead. \cite{detox2019} interpolates between \draco{} and robust aggregation methods for faster computation on both compute nodes and the PS. However, it does not mitigate the communication bottleneck, whereas \solon{} introduces both black-box Byzantine-resilience guarantee and communication-efficiency.  

Communication-efficient distributed machine learning has gained a lot of attention. Various methods propose to use gradient compression, \eg via quantization~\cite{seide20141,alistarh2016qsgd,wen2017terngrad,suresh2017distributed} or sparsification~\cite{stich2018sparsified,Wang18Atomo,lin2017deep,vogels2019powersgd,agarwal2020accordion} to enhance the communication efficiency. These methods massively compress the gradients, however, their Byzantine-resilience is not clear. 

The methods that are the most similar to \solon{} are \signum{}~\cite{bernstein2018signsgd} and the one proposed in~\cite{ghosh2020communication}. These methods introduce both communication-efficiency and Byzantine-resilience, however their Byzantine-resilience guarantees are not as strong as for \solon{} in theory, i.e. they typically use lossy compression for coding and decoding schemes, which only achieve approximated recovery under certain attacks. 
\cite{communciation_gradcoding_min_ye} considers the trade-offs between communication efficiency and straggler tolerance. 
On the other hand, our work focuses on improving communication efficiency in a Byzantine-aware distributed system.  



==> Solon_Arxiv (5)/Theory.tex <==
\section{\solon{}}
\label{sec:solon}

In this section we give an overview of the \solon{} framework, discuss constraints on the encoding and decoding functions, and define optimal coding schemes.

The proofs are left to the appendix.
\subsection{Preliminaries}	
\paragraph{Basic notations.}
For a matrix $\mathbf{A}$, let $\mathbf{A}_{i,j}$, $\mathbf{A}_{i,\cdot}$, and $\mathbf{A}_{\cdot, j}$ denote entries, rows, and columns, respectively. More generally, $\mathbf{A}_{S,T}$ is the submatrix of $\mathbf{A}$ with rows indexed by  $S$ and columns indexed by $T$. The Hadamard, or elementwise, product $\mathbf{A} \odot \mathbf{B}$ of two matrices of the same size has entries $(\mathbf{A}\odot \mathbf{B})_{i,j} = \mathbf{A}_{i,j}\mathbf{B}_{i,j}$. Let $m$ be the dimension of the data, $n$ be the size of the training set, and $\mathbf{x}_i\in\mathbb{R}^m$, $i=1,\ldots,m$ be the data points. Let $\ell(\cdot;\cdot)$ be the loss function, $d$ be the model dimension, and ${\bf w}\in\mathbb{R}^d$ be the model parameters.  Let $\mathbf{1}_m$ and $\mathbf{1}_{n\times m}$ be the $m\times 1$ vector, and $n\times m$ matrix, of all ones, respectively. Similarly, let $\mathbf{0}_{m}, \mathbf{0}_{n\times m}$ contain zeros.  The empirical risk minimization (ERM) \cite{NIPS1991ERM,vapnik2013nature} objective is: 
$\min_{{\bf w}} {n}^{-1}\sum_{i=1}^n \ell({\bf w};\mathbf{x}_i).$
The most common current approach is to use first-order stochastic optimization to solve this, in particular mini-batch stochastic gradient descent (SGD). Starting at an initial point ${\bf w}_0$, we iterate 
${\bf w}_k = {\bf w}_{k-1} - \gamma/|S_k| \sum_{i \in S_k}\nabla\ell_{\bf w}({\bf w}_{k-1}; \mathbf{x}_{i}),$
where $S_k \subseteq \{1,\ldots, n\}$ is a random subset of size $B$ and $\gamma>0$ is the learning rate.

We relabel $S_k$ to $\{1,\ldots, B\}$ and denote $\nabla \ell({\bf w}_{k-1};\mathbf{x}_i)$ by $\mathbf{g}_i$. 

\paragraph{Distributed learning.}
We aim to compute $\mathbf{g}=\sum_{i = 1}^B \mathbf{g}_i$ in a distributed, {\it adversary-resistant}, and {\it communication efficient} manner. We consider a distributed training model where gradient computations are partitioned across $P$ compute nodes at each iteration. These operate on a potentially reduced dimension $d_c$ for communication efficiency, and we let the gradient \emph{compression ratio} be $\smash{r_c \triangleq d/d_c}$. After computing and summing up their assigned gradients, each node sends their answer back to the parameter server (PS). This sums them and updates the model. By applying \solon{}, we reduce the communication complexity for sending gradients to server from $\mathcal{O}(Pd)$ to $\mathcal{O}(Pd_c)$. The broadcast phase of sending aggregated gradients from server to compute nodes takes $\mathcal{O}(\log{(P)}d)$, which is not the major overhead. 

We assume that at most $s$ compute nodes are unreliable, Byzantine, or adversarial, and can send to the PS an arbitrary update. 
We consider the strongest possible adversaries: with infinite computational power, knowing the entire data set, the training algorithm, any defenses present in the system, and able to collaborate.

\subsection{Framework}	\vspace{-0.1in}
\solon{} is defined by the tuple, or \emph{mechanism}, $(\mathbf{A}, E, D)$, where $\mathbf{A}$ is an allocation matrix specifying how to assign gradients to nodes, $E$ are encoding functions determining how each compute node should locally encode its gradients, and $D$ is a decoding function determining how the PS should decode the output of the nodes. As an example, in Figure \ref{fig:RunningExample}(a), $A$ corresponds to the gradient computation assignment of the compute nodes, $E$ corresponds to the summation of the gradients by each node, and $D$ refers to the decoding phase at the PS. 
We generalize the scheme in Figure \ref{fig:RunningExample} to $P$ compute nodes and $B$ gradients. 

{\bf Allocation matrix, $\mathbf{A}$.} 
At each iteration of the training process, we assign the $B$ gradients to the $P$ compute nodes using a $P\times B$ {\it allocation matrix} $\mathbf{A}$, where $\mathbf{A}_{j,k}$ is equal to unity ("1") if node $j$ is assigned to the $k$th gradient ${\bf g}_k$, and zero ("0") otherwise. The support of $\mathbf{A}_{j,\cdot}$, denoted $\supp\left(\mathbf{A}_{j,\cdot}\right)$, is the set of indices of gradients evaluated by the $j$th node. For simplicity, we will assume $B=P$. % throughout the following.
Let $\|\mathbf{A}\|_0$ be to the $L_0$ norm of a matrix, i.e., the number of nonzero entries.
Following \cite{DRACO}, we define the \emph{redundancy ratio} of an allocation as the average number of gradients assigned to each compute node, or equivalently $r\triangleq  \|\mathbf{A}\|_0/P$.

We define the $d \times P$ matrix $\mathbf{G}$ with gradients as its columns: $\mathbf{G} \triangleq [\mathbf{g}_1,\mathbf{g}_2,\cdots, \mathbf{g}_P]$. The $j$th node first picks out its assigned gradients using the allocation matrix $\mathbf{A}$, computing a $d\times P$ gradient matrix $\smash{\mathbf{Y}_j \triangleq \left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}}$. 
The columns of this matrix are $\mathbf{g}_k$ if the $k$th gradient $\mathbf{g}_k$ is allocated to the $j$th compute node, \ie $\mathbf{A}_{j,k} \not = 0$, and zero otherwise.

{\bf Encoding Functions, $E$.} The $j$th compute node is equipped with an encoding function $E_j$ that maps the $d\times P$ matrix $\mathbf{Y}_j$ of its assigned gradients to a $d_c$-dimensional vector.
The $j$th compute node computes and sends $\smash{\mathbf{z}_j \triangleq E_j(\mathbf{Y}_j)}$ to the PS.
If the $j$th node is adversarial, then it instead sends $\smash{\mathbf{z}_j+\mathbf n_{j}}$ to the PS, where $\mathbf n_{j}$ is an arbitrary $d_c$-dimensional \emph{Byzantine} vector.
We let  $E = \{ E_1, E_2, \cdots, E_P\}$ be the set of local encoding functions.

{\bf Decoding Function, $D$}. The $d_c \times P$ matrix $\smash{\mathbf{Z}=\mathbf{Z}^{\mathbf{A},E,\mathbf{G}} \triangleq [\mathbf{z}_1, \mathbf{z}_2,\cdots, \mathbf{z}_P]}$ contains all outputs of the nodes. The $d_c \times P$ matrix $\smash{\mathbf{N} \triangleq [\mathbf{n}_1, \mathbf{n}_2,\cdots, \mathbf{n}_P]}$ contains all Byzantine vectors, with at most $s$ non-zero columns.
Then, the PS receives a $d_c\times P$ matrix $\smash{\mathbf{R} \triangleq \mathbf{Z} +\mathbf{N}}$, and computes a $d$-dimensional vector $\smash{\mathbf{u} \triangleq D(\mathbf{R})}$ using a decoding function $D$.

We require that the algorithm at the PS recovers the $d$-dimensional sum of gradients, $\mathbf{G} \mathbf{1}_P$:

\begin{definition}
	\solon{} with $(\mathbf{A}, E, D)$ can tolerate $s$ adversarial nodes, if for any $\mathbf{N} = [\mathbf{n}_1,\mathbf{n}_2,\cdots, \mathbf{n}_P]$ such that $ \left\vert{ \{j:\mathbf{n}_{j}\not=0\} }\right\vert \leq s$, we have $D(\mathbf{Z}+\mathbf{N}) = \mathbf{G}\mathbf{1}_P$.
\end{definition}

If we defend against the Byzantine attack, then the model update at each iteration is identical to the adversary-free setting. 
This implies that  convergence guarantees for the adversary-free case transfer to the adversarial case.

\subsection{Encoding and decoding functions}	\vspace{-0.1in}
What are the fundamental limits of the above allocation, encoding, and decoding schemes, in particular of the redundancy ratio used in allocation and the compression ratio used in encoding?  Perhaps surprisingly, \emph{the redundancy ratio does not depend on the compression ratio}.
The encoded gradients at each compute node can be arbitrarily compressed without affecting the our ability to tolerate Byzantine attacks.
The reason is that any $d$-dimensional real vector can be mapped one-to-one to a real number. This is stated in the following theorem.

\begin{theorem}\label{Thm:GenericBound}
	If there is a mechanism $(\mathbf{A}, E, D)$ of gradient allocation, encoding, and decoding with redundancy ratio $r$ tolerating $s$ adversarial nodes with a compression ratio $r_c$ of unity, then there is a mechanism $(\mathbf{A}', E', D')$ with redundancy ratio $r$ tolerating $s$ adversarial nodes for any compression ratio $r_c>0$.
\end{theorem}


However $(\mathbf{A}', E', D')$ is in a sense pathological and it is unclear if it can reduce the the number of bits communicated.
Therefore, we seek classes of \textit{regular} encoder and decoder functions $E,D$, to reduce communication cost.

\begin{definition}
	 A set of encoding functions $E$ is called {\em regular} if each output element of each function $E_j$ is a function of linear combinations of columns of the input. Formally, if $E_{j,v}$ is the $v$th element of $E_j$, then
	 $(\mathbf{A}, E, D)$ is regular if there exists a $d\times P$ matrix $\mathbf{U}_{j,v}$ and functions $\smash{\hat{E}_{j,v}}$, such that $\smash{E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}\left(\mathbf{1}_d^T\left(\mathbf{U}_{j,v} \odot \mathbf{Y}_{j}\right)\right)}$.
\end{definition}

When $d=1$, $\mathbf{Y}_j$ has only one row and $\mathbf{1}_{d}=1$ is a scalar.
Thus, $E_{j,v}(\mathbf{Y}_j) = \hat{E}_{j,v}(\mathbf{U}_{j,v} \odot \mathbf{Y}_j)$ implies that $E$ is an arbitrary function of $\mathbf{Y}_j$.
When $d>1$, each output coordinate only depends on linear combinations of input columns.
Since linear combinations do not introduce extra bits, this allows practical communication compression. We will study regular encoders $E$.

\paragraph{Redundancy Bound.}
We first study redundancy requirements for exact recovery of the sum of gradients with $s$ adversaries and compression ratio $r_c$. 
\begin{theorem}\label{Thm:RedundancyRatioBound}
A mechanism $(\mathbf{A}, E, D)$ of gradient allocation, regular encoding, and decoding with compression ratio $r_c$ tolerating $s$ adversarial nodes must have a redundancy ratio $r \geq 2s+r_c$.
\end{theorem}

Thus, for any regular encoder, each gradient has to be replicated on average at least $2s+r_c$ times to defend against $s$ adversarial nodes with a communication compression ratio of $r_c$. If a mechanism tolerates $s$ adversarial nodes with a communication compression ratio of $r_c$, by Theorem \ref{Thm:RedundancyRatioBound}, each compute node encodes at least $(2s+r_c)$ $d$-dimensional vectors on average. If the encoding has linear time complexity, then each encoder requires $O((2s+r_c)d)$ operations in the worst case. If the decoder $D$ has linear time complexity, then it requires at most $O(Pd_c)$ operations in the worst case, as it needs to use the $d$-dimensional input from all $P$ compute nodes. This gives a computational cost of $O(Pd_c)$, which is less than the bound $\mathcal{O}(Pd)$  for the repetition code in \cite{DRACO}.

To better understand the lower bound, we give an equivalent formulation it in the language of linear algebra. Let $g$ be one of the $d\times 1$ dimensional gradients. Suppose it gets sent to $r$ nodes. Then the potentially  corrupted output of the linear encoder at each node $j$  can be represented by $R_j = Z_j g + n_j$, and $n_j$ is the noise here for $j=1,\ldots, r$, where each $Z_j$ is a $d_c \times d$ dimensional matrix. If the number of adversaries is at most $s$, then at most $s$ vectors $n_j$ are nonzero. We call this set of perturbation $B_{s,r}$. Thus, the goal is to design the $r$ matrices $Z_j$, such that for any collection of vectors $n_j$ at most $s$ of which are nonzero, it is possible to recover $g$ from the observations $(Z_j,r_j)$, $j=1,\ldots, r$.
Let $R:=(R_1,\ldots, R_r)$ and $n:=(n_1,\ldots,n_r)$, which we view as a concatenation of vectors belonging to the allowed set $B_{s,r}$. For the recovery of $g$ to be possible, we need that if $R(g,n) = R(g',n')$ for $g,g'\in \R^d$ and $n,n'\in B_{s,r}$, then $g=g'$. 

We can write $R$ as a linear function $R = Zg+n$, where $Z$ is an $rd_c\times d$ concatenation of the matrices $Z_i$. Thus, we can write $R(g,n) = R(g',n')$ as
$Zg+n=Zg'+n' \iff Z(g-g')=n-n'.$
Moreover, we have $n''  = n-n' \in B_{2s,r}$, because at  most $2s$ of its $P$ sub-vectors of size $d_c$ are nonzero. Clearly, all vectors in $B_{2s,r}$ can be written in this form.  Denoting $x = g-g'$, the problem is to understand when there exists a matrix $Z$ such that for all $x \in \R^d$, we have $Zx \notin B_{2s,r}$. Now, $B_{2s,r}$ is a union of several $2sd_c$-dimensional linear subspaces in $rd_c$ dimensions. Moreover, $Zx$ belongs to $span(Z)$, which is an at most $d$-dimensional subspace in $rd_c$ dimensions. Thus, for this to be possible, by counting dimensions we obtain that we need $rd_c\ge 2sd_c +d$. Since $r_c=d/d_c$, this is equivalent to $r\ge 2s +r_c$. This finishes the proof of the fundamental lower bound on the redundancy.



\subsection{Optimal Coding Schemes}
\label{ocs}
%\paragraph{Optimal Coding Schemes}
	\vspace{-0.1in}
Can we achieve the optimal redundancy bound with linear-time encoding and decoding? 
More formally, can we design a tuple $(\mathbf{A},E,D)$ with redundancy ratio $r=2s+r_c$ and computation complexity $\mathcal{O}((2s+r_c)d)$ at the compute nodes and $\mathcal{O}(Pd_c)$ at the PS?
We give a positive answer by designing certain {\em linear block codes} that match the above bounds. 

This is a challenging problem. In fact, we can show (see Appendix \ref{sp}) that this question is \emph{exactly equivalent to a sparse recovery problem}, where we wish to recover an unknown sparse vector from linear combinations of a fixed set of vectors \cite{chen1994basis,chen2001atomic,elad2010sparse}. 
With this lens, our algorithms are related to the classical Prony's method in signal processing \cite{hurst1987scattering,Prony}. However, a key difference is that in our case, we have a \emph{structured set of perturbations}, where entire sub-vectors corresponding to gradients are perturbed at the same time. We leverage this to develop algorithms faster than Prony's method.
\vspace{-0.1in}
\paragraph{Linear Block Code.} 
%Now we introduce a class of linear block code.
We focus on the case when $2s+r_c$ divides $P$; otherwise we can change $P$ or $r_c$ until $2s+r_c$ divides $P$. 
Divide the compute nodes into $q:=P/(2s+r_c) = P/r$ ``blocks'' or groups.
We assign each node in the same block to compute the same gradients. 
Each node sends some linear combination of coordinates of the assigned gradients to the PS (``linear'').
The PS solves systems of linear equations to get the desired gradient sum.  
Following the convention of coding theory \cite{abclbc}, we call our approach \textit{linear block codes}.

The linear block code $(\mathbf{A}, E, D)=(\mathbf{A}^{LBC}, E^{LBC}, D^{LBC})$ is defined as follows. 
The assignment matrix is $\mathbf{A} = \mathbf{I}_q \otimes \mathbf{1}_{r \times r}$.

The $j$th compute node first selects its allocated gradients $\mathbf{Y}_j=\left( \mathbf{1}_d \mathbf{A}_{j,\cdot} \right)\odot \mathbf{G}$.
Its encoder function sums up the allocated gradients into $\mathbf{Y}_j \mathbf{1}_P$, then computes and sends $\mathbf{z}_j = E_j(\mathbf{Y}_j) = \mathbf{W}_j \mathbf{Y}_j\mathbf{1}_P$  to the PS, where $\mathbf{W}_j$ is a $d_c \times d$ matrix. 

The decoder function, summarized in Algorithm \ref{Alg:DecoderFunction_LinearBlock}, partitions the received updates into the $q$ blocks computing identical gradients.
For each, a block decoder $\psi(\cdot,\cdot)$ is called to recover the sum of all gradients in this group.
\begin{algorithm}[htbp]
	\SetKwInOut{Input}{Input}
	\SetKwInOut{Output}{Output}
	\Input{Received $d_c \times P$ matrix $\mathbf{R}$}
	\Output{Desired gradient summation $\mathbf{u}$}
	Let $\mathbf{R} = \left[\mathbf{R}_1, \mathbf{R}_2, \cdots, \mathbf{R}_{q}\right]$, where each $\mathbf{R}_j$ is a $d_c\times r $ matrix
	
    \For{$j=1$ \KwTo $q$ }
    {
         \textrm{ } $ V = \phi(\mathbf{R}_j,j)$ // Locate the adversarial nodes\\
		$U = \{1,2,\cdots,r\} \setminus V$ // Non-adversarial nodes\\
    $\mathbf{u}_j = \psi(\mathbf{R}_j,j, U)$ // Decode each block using the non-adversarial nodes
    }
	%into $d_c\times r$ matrices
	Compute and return $\mathbf{u} = \sum_{i=1}^{q}\mathbf{u}_i$
	\caption{Decoder Function $D$.}
	\label{Alg:DecoderFunction_LinearBlock}
\end{algorithm}

There are three questions left: (i) how $\mathbf{W}_j$ is constructed, (ii) how the adversarial node index location function $\phi(\cdot)$ works, and (iii) how the block decoder function $\psi(\cdot,\cdot)$ works.

Given any distinct nonzero scalars $w_1, w_2, \cdots, w_P$, we propose to construct $\mathbf{W}_j$ as $\mathbf{W}_j \triangleq \mathbf{I}_{d_c}\allowbreak$ $\otimes [\allowbreak1,\allowbreak w_j,\allowbreak w_j^2,\allowbreak \cdots,\allowbreak w_j^{r_c-1}]$. The adversarial node index locating function $\phi(\cdot)$ works as follows.
Given the $d_c \times r$ matrix $\mathbf{R}_j$ received from the compute nodes, we first generate a $1\times d_c$ random vector $ \mathbf{f} \sim \mathcal{N}(\mathbf{1}_{1\times d_c},\,\mathbf{I}_{d})$,
and then compute $\smash{\mathbf{r}_{j,c} \triangleq \mathbf{f} \mathbf{R}_j}$.
Next, we obtain an $r$-dimensional vector $\mathbf{a} = [a_1, a_2,\cdots, a_{r}]$ by  solving the linear system
$\begin{bmatrix}
     \hat{\mathbf{W}}_{j,r_c+s-1},\allowbreak  & -\hat{\mathbf{W}}_{j,s-1} \odot\allowbreak \left( \mathbf{r}_{j,c}^T \mathbf{1}_{s}^T\right)
\end{bmatrix}
    \mathbf{a}= \mathbf{r}_{j,c} \odot \left[\hat{\mathbf{W}}_{j,s}\right]_{\cdot,s}$,
 where 
	\[
\hat{\mathbf{W}}_{\mathit{j},v} \triangleq
\begin{bmatrix}
1 & w_{(j-1)r+1} &  w_{(j-1)r+1}^2 &\cdots &  w_{(j-1)r+1}^{v} \\
1 & w_{(j-1)r+2} &  w_{(j-1)r+2}^2 &\cdots &  w_{(j-1)r+2}^{v} \\
\vdots & \vdots & \vdots & \vdots & \vdots\\
1 & w_{jr} &  w_{jr}^2 &\cdots &  w_{jr}^{v}
 \\
\end{bmatrix}.
\\
\]
Finally compute $P_j(w) \triangleq (\sum_{i=0}^{r_c+s-1} a_{i+1} w^i)/(w^s+\sum_{i=0}^{s-1} a_{i+r_c+s+1} w^i) $,
and return $V=\{i|P_j(w_{(r-1)j+i}) \not =\left[ \mathbf{r}_{j,c}\right]_i\}$.
The decoding function $\psi(\cdot, \cdot)$ computes and returns $\textit{vec}\left(\left[\mathbf{R}_{j}\right]_{\cdot, U} \left[\hat{W}_{j,r_c-1}\right]_{U,\cdot}^{-1,T}\right)$ given the non-adversarial node indices $U$.

The following lemma ensures that the Byzantine nodes are correctly found.
\begin{lemma}\label{Thm:LBCDetection}
	Suppose $\left\vert{\{j:\|\mathbf{n}_{j}\|_0 \not=0\}}\right\vert$ $\leq s$ and $r\geq r_c+2s$. 
	Then $\phi(\mathbf{R}_j,j) =  \{i:\|\mathbf{n}_{j(r-1)+i}\|_0 \not=0\}$ with probability equal to unity. 
\end{lemma}
The next lemma demonstrates that within each group the gradient is correctly recovered.
\begin{lemma}\label{thm:LBClocalcorrect}
	If $U$ consists solely of at least $r-s$ non-adversarial nodes, then  with probability equal to unity, $\mathbf{u}_j = \sum_{k=(j-1)r+1}^{jr}\mathbf{y}_{k}$.
\end{lemma}

Combing the above two results,  we show that the linear block code tolerates any $s$ adversaries, achieving the optimal redundancy and compression ratio with linear-time encoding and decoding.

\begin{theorem}\label{Thm:LinearBlockCodeOptimality}
	The linear block code  $(\mathbf{A}, E, D)$ tolerates any $s$ adversaries with probability equal to unity, and achieves the redundancy ratio  bound. For $d\gg P$, its encoding and decoding achieve linear-time computational complexity. 
\end{theorem} 

Theorem \ref{Thm:LinearBlockCodeOptimality} shows that the linear block code is information theoretically tight and enjoys a small computational overhead even for large ML models. 


==> Solon_Arxiv (5)/macros.tex <==
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{wrapfig}
\usepackage{bbm}
\usepackage{hyperref}       % hyperlinks
\usepackage{url}            % simple URL typesetting
\usepackage{booktabs}       % professional-quality tables
\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{amsthm,amsmath,amssymb}
%\usepackage{graphicx,xspace,verbatim,comment}
%\usepackage{array,color,multirow}
%\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{float,url,amsfonts,alltt}
\usepackage{mathtools,rotating}
\usepackage{ifpdf,fancyvrb}
\usepackage{enumitem}
%\usepackage{algorithm,algpseudocode}
%\usepackage{etoolbox,listings,subcaption}
%\usepackage{bigstrut,morefloats}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
%\usepackage{thm-restate}
%\usepackage{todonotes}
%\usepackage[boxruled]{algorithm2e}
%\usepackage{pbox}
\usepackage{subfigure}
% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
%\usepackage{subfigure}
\usepackage{booktabs} % for professional tables
\usepackage{hyperref}

\usepackage{graphicx,xspace,verbatim,comment}
\usepackage{hyperref,array,color,balance,multirow}
\usepackage{balance,float,url,amsfonts,alltt}
\usepackage{mathtools,rotating,amsmath,amssymb}
\usepackage{color,ifpdf,fancyvrb,array}
% \usepackage{algorithm,algpseudocode}
\usepackage{etoolbox,listings}
%\usepackage{subcaption}
\usepackage{bigstrut,morefloats}
\usepackage{makecell}
%\usepackage[boxruled]{algorithm2e}
\usepackage{pbox}
\usepackage[numbers]{natbib}
\usepackage{algorithm, algorithmic}
\usepackage[boxruled,algo2e,linesnumbered]{algorithm2e}
\DeclarePairedDelimiterX{\inp}[2]{\langle}{\rangle}{#1, #2}

\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{remark}{Remark}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{definition}{Definition}
\newcommand{\eat}[1]{}

\newcommand{\gaussian}[2]{\mathcal{N}(#1,#2)}


% User Defined Commands
\newcommand{\systemnameSolon}{\textsc{Solon}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\cmp}{\mathbb{C}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\detox}{\textsc{Detox}}
\newcommand{\draco}{\textsc{Draco}}
\newcommand{\solon}{\textsc{Solon}}
\newcommand{\bulyan}{\textsc{Bulyan}}
\newcommand{\multikrum}{\textsc{Multi-Krum}}
\newcommand{\signum}{\textsc{Signum}}
% \newcommand{\eg}{\textit{e.g., }}
% \newcommand{\ie}{\textit{i.e., }}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\hier}{\textsc{Hier-Aggr}}
%
\newcommand{\lingjiao}[1]{{\color{blue} {\bf Lingjiao:} #1}}
\newcommand{\leshang}[1]{{\color{red} {\bf Note:} #1}}

\newcommand{\sgn}{\operatorname{sign}}
\newcommand{\indi}{\mathds{1}}
\newcommand{\ie}{{\emph i.e.,} }
\newcommand{\eg}{{\it e.g.}, }
\newcommand{\tr}{\operatorname{tr}}
% \newcommand{\R}{\mathbb{R}}
%\newcommand{\C}{\mathbb{C}}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\var}{\operatorname{Var}}
\newcommand{\card}{\operatorname{card}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\cov}{\operatorname{Cov}}
% \newcommand{\PP}{\mathbb{P}}
\newcommand{\vecx}{\mathbf{x}}
\newcommand{\vecw}{\mathbf{w}}
\newcommand{\vecwb}{\mathbf{w}}
\newcommand{\tvecw}{\widetilde{\mathbf{w}}}
\newcommand{\tvecwb}{\widetilde{\mathbf{w}}}
\newcommand{\vecv}{\mathbf{v}}
\newcommand{\ovecv}{\overline{\mathbf{v}}}
\newcommand{\vecy}{\mathbf{y}}
\newcommand{\vecg}{\mathbf{g}}
\newcommand{\vecr}{\mathbf{r}}
\newcommand{\veca}{\mathbf{a}}
\newcommand{\vecb}{\mathbf{b}}
\newcommand{\vecn}{\mathbf{n}}
\newcommand{\vece}{\mathbf{e}}
\newcommand{\vecz}{\mathbf{z}}
\newcommand{\tvecz}{\widetilde{\mathbf{z}}}
\newcommand{\matA}{\mathbf{A}}
\newcommand{\matP}{\mathbf{P}}
\newcommand{\matD}{\mathbf{D}}
\newcommand{\matX}{\mathbf{X}}
\newcommand{\gradf}{\nabla f}
\newcommand{\tf}{\widetilde{f}}
\newcommand{\gradtf}{\nabla \widetilde{f}}
\newcommand{\gradF}{\nabla F}
\newcommand{\HW}{\textsc{Hogwild!}}
\newcommand{\setS}{\mathcal{S}}
\newcommand{\matS}{\mathbf{S}}
\newcommand{\const}{\mathcal{O}(1)}
\newcommand{\bigo}{\mathcal{O}}
\newcommand{\setI}{\mathcal{I}}
\newcommand{\CM}{\textsc{KroMagnon}}
\newcommand{\cdeg}{\overline{\Delta}}
\newcommand{\ct}{\mathcal{O}(1)}
\newcommand{\W}{\mathcal{W}}
\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\mat}[1]{\mathbf{#1}}
\newcommand{\norm}[1]{\left\|#1\right\|}
\newcommand{\norms}[1]{\|#1\|}
\newcommand{\twonm}[1]{\left\|#1\right\|_2}
\newcommand{\twonms}[1]{\|#1\|_2}
\newcommand{\onenm}[1]{\left\|#1\right\|_1}
\newcommand{\onenms}[1]{\|#1\|_1}
\newcommand{\fbnorm}[1]{\left\|#1\right\|_F}
\newcommand{\fbnorms}[1]{\|#1\|_F}
\newcommand{\prob}[1]{\mathbb{P}\left\{#1\right\}}
\newcommand{\probs}[1]{\mathbb{P}\{#1\}}
\newcommand{\EXP}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\EXPS}[1]{\mathbb{E}[#1]}
\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
\newcommand{\innerp}[2]{\left\langle#1,#2\right\rangle}
\newcommand{\innerps}[2]{\langle#1,#2\rangle}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\abss}[1]{|#1|}
\newcommand{\tsp}{^{\rm T}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}
\newcommand{\mt}{B\floor{t/B}}
%\newcommand{\G}{\overline{G}}
%\newcommand{\B}{\overline{B}}
\numberwithin{equation}{section}
\newcommand{\eq}[1]{(\ref{eq:#1})}
\newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
\newcommand{\red}[1]{{\color{red}{#1}}}

\newcommand{\paris}[1]{{\color{red} #1}}


\newcommand\overmat[2]{%
	\makebox[0pt][l]{$\smash{\color{white}\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{\color{black}#1}}}$}#2}
\newcommand\bovermat[2]{%
	\makebox[0pt][l]{$\smash{\overbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}^{\text{#1}}}$}#2}
					
\newcommand\bundermat[2]{%
	\makebox[0pt][l]{$\smash{\underbrace{\phantom{%
					\begin{matrix}#2\end{matrix}}}_{\text{#1}}}$}#2}
					
					
\newcommand\partialphantom{\vphantom{\frac{\partial e_{P,M}}{\partial w_{1,1}}}}

\newcommand{\scream}[1]{{\bf * #1 *}{\typeout{#1}}}

\usepackage{amsmath}
\usepackage{accents}
\newlength{\dhatheight}
\newcommand{\doublehat}[1]{%
    \settoheight{\dhatheight}{\ensuremath{\hat{#1}}}%
    \addtolength{\dhatheight}{-0.35ex}%
    \hat{\vphantom{\rule{1pt}{\dhatheight}}%
    \smash{\hat{#1}}}}
    
%\usepackage{algorithm,algpseudocode}


\newtheorem{theo}{Theorem}
\newtheorem{introtheo}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{dfn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}{Corollary}
\newtheorem{rem}{Remark}
\newtheorem{asm}{Assumption}
\newtheorem{example}{Example}
\newtheorem{property}{Property}

\newcommand{\blkdiag}{\text{blkdiag}}
\newcommand{\GGG}{{\color{red}{\bf [GGG CHECK]}}}
\newcommand{\sort}{\text{sort}}
\newcommand{\Span}{\text{span}}
\newcommand{\supp}{\text{supp}}
\newcommand{\bsp}{\hspace{-0.14cm}}
\newcommand{\T}{\intercal}
\newcommand{\eqdef}{\stackrel{\triangle}{=}}
\newcommand{\G}{ \mathcal{G} } 
\newcommand{\Gnp}{ \mathcal{G}\left(n,\frac{1}{2}\right) } 
\newcommand{\Gnpk}{ {G}\left(n,\frac{1}{2}, k\right) }
\newcommand{\opt}{\textsf{opt}}
\newcommand{\A}{{\bf A}}
\newcommand{\den}{\textsf{den}}
\usepackage[T1]{fontenc}
\usepackage{upgreek}

\newcommand{\Exp}{\mathbb{E}}
\usepackage[greek,english]{babel}
% \usepackage[utf8x]{inputenc}
\usepackage{pifont}
\usepackage{float}
\usepackage{autobreak}

